Learning Fair Node Representations with Graph Counterfactual Fairness

Fair machine learning aims to mitigate the biases of model predictions against certain subpopulations regarding sensitive attributes such as race and gender. Among the many existing fairness notions, counterfactual fairness measures the model fairness from a causal perspective by comparing the predictions of each individual from the original data and the counterfactuals. In counterfactuals, the sensitive attribute values of this individual had been modified. Recently, a few works extend counterfactual fairness to graph data, but most of them neglect the following facts that can lead to biases: 1) the sensitive attributes of each node's neighbors may causally affect the prediction w.r.t. this node; 2) the sensitive attributes may causally affect other features and the graph structure. To tackle these issues, in this paper, we propose a novel fairness notion - graph counterfactual fairness, which considers the biases led by the above facts. To learn node representations towards graph counterfactual fairness, we propose a novel framework based on counterfactual data augmentation. In this framework, we generate counterfactuals corresponding to perturbations on each node's and their neighbors' sensitive attributes. Then we enforce fairness by minimizing the discrepancy between the representations learned from the original graph and the counterfactuals for each node. Experiments on both synthetic and real-world graphs show that our framework outperforms the state-of-the-art baselines in graph counterfactual fairness, and also achieves comparable prediction performance.

==> body.tex <==
%\section{Nonsense}
%The key of group fairness is ``some individuals in different sensitive subgroups should be treated equally''. Here ``equal'' often be formally defined as ``the distributions of predictions in each counterpart group should be the same'', i.e., $$P(\hat{Y}|S=0)=P(\hat{Y}|S=1)$$, or 
%$$ \hat{Y} \bigCI S$$ 





==> fmvmfnbbgqzmgyncbhqsqqzvbvfhfcxv/body.tex <==
%\section{Nonsense}
%The key of group fairness is ``some individuals in different sensitive subgroups should be treated equally''. Here ``equal'' often be formally defined as ``the distributions of predictions in each counterpart group should be the same'', i.e., $$P(\hat{Y}|S=0)=P(\hat{Y}|S=1)$$, or 
%$$ \hat{Y} \bigCI S$$ 





==> fmvmfnbbgqzmgyncbhqsqqzvbvfhfcxv/exp.tex <==
\section{Experiments}
We evaluate the proposed method on both synthetic and real-world graphs. The detailed statistics of these datasets are shown in Table~\ref{tab:dataset}, including the number of nodes, the number of edges, the dimension of features, the average degree, and the number of intra-group and inter-group edges with respect to the sensitive attribute.
\begin{table}[t]
%\small
  \caption{Detailed statistics of the datasets.}
  \label{tab:datasets}
 \vspace{-3mm}
  \label{tab:dataset}
  \begin{tabular}{llll}
    \toprule
    Dataset & Synthetic & Bail & Credit\\
    \midrule
    $|\mathcal{V}|$ & $2,000$ & $18,876$ & $30,000$\\ 
    $|\mathcal{E}|$ & $4,120$ & $311,870$ & $137,377$\\ 
    Feature dimension & $26$ & $18$& $13$\\
    Average degree & $5.120$& $34.044$ &$10.158$\\
    \# of intra-group edges & $2,379$ & $162,821$& $120,750$\\
    \# of inter-group edges & $1,741$ &$149,049$& $16,627$\\
    %$R^2(\tilde{S},Y)$ &&&\\
  \bottomrule
\end{tabular}
\vspace{-4mm}
\end{table}

\begin{table*}[t]
\small
\centering
 \caption{Comparison of the performance of node representation learning methods with respect to prediction and fairness.}
 \vspace{-2mm}
 \label{tab:baseline}
 \begin{tabular}{l||l||c|c|c||c|c|c|c}
 \hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{3}{c||}{Prediction Performance} & \multicolumn{4}{c}{Fairness}                     \\\cline{3-9}
                         &                         & Accuracy ($\uparrow$)   & F1-score ($\uparrow$)   & AUROC ($\uparrow$)  & $\triangle_{EO}$ ($\downarrow$) & $\triangle_{DP}$ ($\downarrow$) & $\delta_{CF}$ ($\downarrow$) & $R^2$ ($\downarrow$)\\
\hline
Synthetic                   & GCN  &   $0.686 \pm 0.015$         &  $0.687 \pm 0.020$          &  $0.758 \pm 0.017$    &  $0.050 \pm 0.030$          &   $0.060 \pm 0.033$               &     \underline{$0.101 \pm 0.030$}          & $0.085 \pm 0.050$  \\
                         & GraphSAGE  &   \underline{$0.712 \pm 0.012$}         &  \underline{$0.714 \pm 0.021$}          &  \underline{$0.789 \pm 0.018$}    &   $0.049 \pm 0.036$         &   $0.053 \pm 0.042$               &   $0.172 \pm 0.056$ &   $0.011 \pm 0.011$           \\
                          & GIN   & $0.682 \pm 0.021$            &   $ 0.691 \pm 0.022$         &  $0.741 \pm 0.021$    &  $0.077 \pm 0.053$          &  $0.081 \pm 0.055$               &  $0.301 \pm 0.080$  &    $0.011 \pm 0.009$          \\
                         & C-ENC      &  $0.665 \pm 0.023$          & $0.671\pm 0.031$           & $0.732\pm 0.028$     &  \underline{$0.030\pm 0.024$}          &   \underline{$0.048\pm 0.026$}               &  $0.633\pm 0.013$     &$0.085\pm 0.016$           \\
                         & FairGNN  &  $0.668\pm 0.020$           &  $0.672\pm 0.026$          & $0.735\pm 0.022$     &  \bm{$0.025\pm 0.021$}          &   \bm{$0.042\pm 0.033$}               &   $0.678\pm 0.014$   &  $0.091\pm0.021$          \\
                         & NIFTY-GCN & $0.618 \pm 0.035$            &  $0.640 \pm 0.037$          & $0.672 \pm 0.042$     &   $ 0.172 \pm 0.110$         &   $0.199 \pm 0.106$               &   $0.208 \pm 0.090$     &  $0.105 \pm 0.081$        \\
                         & NIFTY-SAGE & $0.664 \pm 0.041$           &   $0.682 \pm 0.073$         &  $0.755 \pm 0.021$    &   $0.031 \pm 0.027$         &     $0.048 \pm 0.027$             &  $0.147 \pm 0.071$   &     \underline{$0.008 \pm 0.005$}        \\
                         & GEAR             &  \bm{$0.718 \pm 0.018$}          &    \bm{$0.724 \pm 0.022$}        &   \bm{$0.793 \pm 0.014$}    &    $0.052 \pm 0.038$        &  $0.064 \pm 0.038$                & \bm{$0.002 \pm 0.002$}          &  \bm{$0.007 \pm 0.006$}     \\
\hline
Bail               & GCN                     &   $0.838\pm 0.017$         &       $0.782\pm0.023$     &   $0.885 \pm 0.018$   &     $0.023 \pm 0.019$       &      $0.075 \pm 0.014$            &  $0.132 \pm 0.059$ &  $0.075 \pm 0.028$              \\
                         & GraphSAGE   &   \bm{$0.854 \pm 0.026$}         &   \bm{$0.804 \pm 0.032$}         &  \bm{$0.905 \pm 0.021$}    &  $0.039 \pm 0.022$          &  $0.086 \pm 0.039$                &  $0.088 \pm 0.047$       &   $0.069 \pm 0.011$      \\
                          & GIN                     &   $0.731 \pm 0.058$         &     $0.656 \pm 0.084$       &   $0.773 \pm 0.069$   &    $0.041 \pm 0.023$        &     $0.065 \pm 0.034$             & $0.143 \pm 0.069$   &    $0.047 \pm 0.036$          \\
                         & C-ENC  & $0.842 \pm 0.047$            &  $0.792\pm 0.014$          &  $0.889\pm 0.033$    & $0.038\pm 0.022$           &   $0.069\pm 0.020$               &    $0.040 \pm 0.025$      &  $0.078\pm 0.024$      \\
                         & FairGNN               &   $0.835\pm 0.024$    &    $0.784\pm 0.021$        & $0.882\pm 0.035$     &   $0.046\pm 0.013$         &   $0.074\pm 0.026$               &  $0.042 \pm 0.032$          &   $0.086 \pm 0.016$   \\
                          & NIFTY-GCN                   &  $0.752 \pm 0.065$          &  $0.669 \pm 0.050$          & $0.799 \pm 0.051$     &   \underline{$0.019 \pm 0.015$}         &     \bm{$0.036 \pm 0.022$}             &   $0.031 \pm 0.017$   &   $0.025 \pm 0.018$         \\
                         & NIFTY-SAGE                   &   $0.823 \pm 0.048$         &  $0.723 \pm 0.103$          &  $0.876 \pm 0.043$    &    \bm{$0.014 \pm 0.006$}        &  \underline{$0.047 \pm 0.015$}                & \underline{$0.013 \pm 0.011$}  &    \underline{$0.044 \pm 0.020$}           \\
         & GEAR             &     \underline{$0.852 \pm 0.026$}     &    \underline{$0.800 \pm 0.031$}        &  \underline{$0.896 \pm 0.016$}    &   \underline{$0.019 \pm 0.023$}         &     $0.058 \pm 0.017$             & \bm{$0.003 \pm 0.002$}    &   \bm{$0.038 \pm 0.012$}          \\
\hline
Credit                         & GCN                     &   $0.698 \pm 0.028$         &   $0.794 \pm 0.027$         &   $0.684 \pm 0.019$   &    $0.087 \pm 0.035$        &    $0.108 \pm 0.031$              &  $0.042 \pm 0.029$ &   $0.022 \pm 0.014$            \\
                         & GraphSAGE                     &  $0.739 \pm 0.009$          &  $0.821 \pm 0.008$          &  \bm{$0.756 \pm 0.011$}    &      $0.094 \pm 0.033$      &     $0.109 \pm 0.030$             &  $0.062 \pm 0.036$   &         $0.014 \pm 0.004$    \\
                          & GIN                     &    $ 0.713 \pm 0.018$        &   $0.805 \pm 0.016$         & $0.706 \pm 0.010$     &    $0.121 \pm 0.042$        &    $0.130 \pm 0.037$              &    $0.123 \pm 0.060$ &   $0.025 \pm 0.012$           \\
                         & C-ENC   &  $0.695\pm 0.011$          &    $0.786\pm 0.012$        & $0.683\pm 0.018$     &   $0.098\pm 0.025$         &  $0.104\pm 0.042$                & $0.100\pm 0.024$    &  $0.048\pm 0.012$           \\
                         & FairGNN                 &   $0.683\pm 0.053$         &   $0.780\pm 0.042$         &  $0.680\pm 0.021$    &    $0.175 \pm 0.035$        &   $0.187\pm 0.036$               &  $0.105\pm 0.053 $   &     $0.056 \pm 0.018$        \\
                         & NIFTY-GCN                   &   $0.697 \pm 0.007$         &  $0.792 \pm 0.007$          &   $0.685 \pm 0.007$   &   $0.097 \pm 0.024$         &  $0.106 \pm 0.021$                & $0.004 \pm 0.004$      &   $0.017 \pm 0.003$        \\
                         & NIFTY-SAGE                   &  \underline{$0.751 \pm 0.023$}          &      \underline{$0.833 \pm 0.020$}  &  $0.730 \pm 0.011$    &  \bm{$0.075 \pm 0.021$}          &   \bm{$0.094 \pm 0.019$}               &  \underline{$0.004 \pm 0.003$}     &     \underline{$0.011 \pm 0.003$}      \\
                         & GEAR            &   \bm{$0.755 \pm 0.011$}         &   \bm{$0.835 \pm 0.008$}         &   \underline{$0.740 \pm 0.008$}   &   \underline{$0.086 \pm 0.018$}         & \underline{$0.104 \pm 0.013$}       &   \bm{$0.001 \pm 0.001$}       &  \bm{$0.010 \pm 0.003$}\\
\hline
\end{tabular}
\vspace{-3mm}
\end{table*}

\vspace{-2mm}
\subsection{Datasets} 
\label{sec:dataset}
A synthetic dataset and two real-world datasets are used in the experiments. In the synthetic dataset, we create a causal model with which we can fully manipulate the data generation process. More specifically, in this synthetic dataset, we generate the features, latent embeddings, graph structure, and labels as below:
\begin{equation}
S_i\sim \text{Bernoulli}(p),\,\, {Z}_i\sim \mathcal{N}(0,\mathbf{I}),\,\, {X}_i=\mathcal{S}({Z}_i) + S_i\mathbf{v},\,\, 
\end{equation}
\begin{equation}
    P({A}_{i,j}=1)\!=\!\sigma(\text{cos}({Z}_i,{Z}_j)+ a\mathbf{1}({S}_i={S}_j)), Y_i=\mathcal{B}(\mathbf{w} Z_i + {w}_s \frac{\sum_{j\in \mathcal{N}_i}S_j}{|\mathcal{N}_i|}),
\end{equation}
% \begin{equation}
% s_i\sim \text{Bernoulli}(p),\,\, \mathbf{z}_i\sim \mathcal{N}(0,\mathbf{I}),\,\, \mathbf{x}_i=\mathcal{S}(\mathbf{z}_i) + s_i\mathbf{v},\,\, 
% \end{equation}
% \begin{equation}
%     p({A}_{ij}=1)\!=\!\sigma(\text{cos}(\mathbf{z}_i,\mathbf{z}_j)+ a\mathbf{1}({s}_i={s}_j)), y_i=\mathcal{B}(\mathbf{w} z_i + {w}_s \frac{\sum_{j\in \mathcal{N}_i}s_j}{|\mathcal{N}_i|}),
% \end{equation}
where we sample the sensitive attribute with Bernoulli distribution, where $p=0.4$ is the probability of $S_i=1$. We sample latent embeddings ${Z}_i \in \mathbb{R}^{d_z}$ from a Gaussian distribution, where $d_z=50$. ${Z}_i$ influences the node features and the graph structure for each node $i$, and $\mathcal{S}(\cdot)$ denotes a sampling operation which randomly selects $d=25$ dimensions out of the latent embeddings to form the observed features ${X}_i$. %so we can infer a part of the latent embeddings from the observed features. 
$\mathbf{v}\in\mathbb{R}^d, \mathbf{v} \sim \mathcal{N}(0,\mathbf{I})$ controls the influence of the sensitive attribute on other features.
%
We simulate the probability of each edge $(i,j)$ based on the cosine similarity between ${Z}_i$ and ${Z}_j$, as well as whether their sensitive attribute values are equal. Here $\mathbf{1}(\cdot)$ is an indicator function which outputs $1$ when the input statement is true and $0$ otherwise. We set parameter $a=0.01$. %between the mean aggregation of neighboring sensitive attribute values $\tilde{S}_i$ and $\tilde{S}_j$. 
Then we sum up the above similarity between $({Z}_i, {Z}_j)$ and the indicator function's output of $(S_i=S_j)$, and map it into a range of $[0,1]$ with a Sigmoid function $\sigma{(\cdot)}$ to compute the link probability between $(i,j)$. %$\|$ here denotes a concatenation operation, and we select top-$25$ nearest neighbors for each node $i$ to form $\mathcal{N}_i$, 
$\mathbf{w}\in \mathbb{R}^{d_z}$ contains parameters sampled from Normal distribution. We average each node's and their one-hop neighbors' sensitive attribute values and use it into label generation with weight ${w}_s=0.5$. In  $\mathcal{B}(\cdot)$, we map $Y_i$ into a binary value. Specifically, we first compute the mean value of $Y_i$ over all nodes, and set $Y_i=1$ if it is larger than the mean value, otherwise $Y_i=0$.

As for the real-world graphs, we use: %1) The \textit{German credit graph} []: In this graph, each node represents a client in a German bank, and each edge represents the  similarity of their credit accounts. We use the clients' gender as the sensitive attribute, and the task is to classify clients into good/bad credit risks. 
1) \textit{Bail} \cite{agarwal2021towards}: This graph contains the data of defendants who got released on bail at the U.S state courts. %during 1990-2009. 
In this graph, each node represents a defendant, each edge between a pair of nodes represents their similarity of criminal records and demographics. We use the defendants' race as the sensitive attribute. The task is to classify defendants into bail (not tend to commit a violent crime if released) or no bail. %(tend to commit a violent crime). 
2) \textit{Credit defaulter} \cite{agarwal2021towards}: This graph contains people's default payment information. In this graph, each node represents an individual, each edge between a pair of nodes represents the similarity of their spending and payment patterns. We use their age as the sensitive attribute, and the task is to predict that their default ways of payment is credit card or not.

% how to generate ground-truth counterfactual data
To evaluate the graph counterfactual fairness of the proposed method, we need to generate the ground-truth counterfactuals with the perturbations on different nodes' sensitive attribute. On the synthetic dataset, the counterfactuals can be generated based on the predefined causal model. On the real-world graphs, the ground-truth causal models are unknown, so we use a simple causal model and fit the observed data, and use the learned parameters in the fitted causal model to generate the counterfactuals for the whole graph. More specifically, we first use a Na\"ive Bayes model to learn $P(X_i|S_i)$, and then update the counterfactual features by $(\mathbf{x}_i)_{S_i\leftarrow{1-s_i}}=\mathbb{E}[{X}_i|S_i=1-s_i]-\mathbb{E}[{X}_i|S_i=s_i]+\mathbf{x}_i$. We use $(\cdot)^{CF}$ to denote any counterfactuals. %for notation simplicity. 
Then we generate the counterfactual graph edge for each $(i, j)$ based on the following rules:
\begin{equation}
    P({A}^{CF}_{i,j}=1)= \sigma(\text{cos}({X}_i^{CF}\backslash S_i^{CF},{X}_j^{CF}\backslash S_j^{CF}) +  \gamma \mathbf{1}({S}^{CF}_i, {S}^{CF}_j)),
\end{equation}
where $\text{cos}(\cdot)$ is cosine similarity. We use $\sigma(\cdot)$ to map its input into a range $[0, 1]$ to compute the link probability for any node pairs in the counterfactual graph.
We fit the data with this causal model and learn the parameter $\gamma$. For evaluation, we use the counterfactual data generated by the causal model and learned parameters. 
%

As discussed in \cite{russell2017worlds}, there might be multiple possible causal models in the real-world data, so we have tried  different causal models to fit the real-world data. Due to the space limit, we only show the results based on the causal model as described above, but the observations over all the experiments are generally consistent.


% \begin{figure}[t]
% \centering
%   \begin{subfigure}[b]{0.22\textwidth}
%         \centering
%         \includegraphics[height=1.in]{figures/lambda.pdf}
%         %\vspace{-2mm}
%         \caption{$\lambda$}
%     \end{subfigure}
%   \begin{subfigure}[b]{0.232\textwidth}
%         \centering
%         \includegraphics[height=1.in]{figures/lambda_s.pdf}
%         %\vspace{-2mm}
%         \caption{$\lambda_s$}
%     \end{subfigure}
%         % \vspace{-2mm}
%   \caption{Parameter study in the Bail dataset.}
%   \label{fig:parameter}
%   %\vspace{-3mm}
% \end{figure}

% \begin{table*}[t]
% \small
% \centering
%  \caption{Comparison of the performance of different subgraph encoders in \mymodel.}
%  \vspace{-2mm}
%  \label{tab:encoder}
%  \begin{tabular}{l||l||c|c|c||c|c|c|c}
%  \hline
% \multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{3}{c||}{Prediction} & \multicolumn{4}{c}{Fairness}                     \\\cline{3-9}
%                          &                         & Accuracy ($\uparrow$)   & F1-score ($\uparrow$)   & AUROC ($\uparrow$)  & $\triangle_{EO}$ ($\downarrow$) & $\triangle_{DP}$ ($\downarrow$) & $\delta_{CF}$ ($\downarrow$) & $R^2$ ($\downarrow$)\\
% \hline
% Synthetic                   & \mymodel-GCN   &     $0.675 \pm 0.018$       &  $0.680 \pm 0.031$          &   $0.749 \pm 0.017$   &  $0.045 \pm 0.036$          &    $0.051 \pm 0.040$              &   $0.003 \pm 0.002$            & $0.010 \pm 0.012$  \\
%             & \mymodel-SAGE            &  $0.718 \pm 0.018$          &   $0.724 \pm 0.022$         &  $0.793 \pm 0.014$    &    $0.052 \pm 0.038$        &  $0.064 \pm 0.038$                & \bm{$0.002 \pm 0.002$ }         &  $0.007 \pm 0.006$     \\
%             & \mymodel-infomax     & $0.669 \pm 0.019$   &    $0.671 \pm 0.035$        & $0.746 \pm 0.018$     &   $0.053 \pm 0.044$         &  $0.056 \pm 0.048$                &   $0.003 \pm 0.001$            &  $0.010 \pm 0.016$ \\
%             & \mymodel-GIN &   $0.676 \pm 0.015$         &   $0.677 \pm 0.026$         &  $0.741 \pm 0.020$    &   $0.033 \pm 0.025$         & $0.055 \pm 0.027$                 &  $0.015 \pm 0.009$             &  $0.009 \pm 0.009$ \\
%             & \mymodel-JK   & $0.682 \pm 0.016$            &  $0.693 \pm 0.025$          &  $0.747 \pm 0.018$    &    $0.065 \pm 0.040$        &               $0.068 \pm 0.050$   &    \bm{$0.002 \pm 0.001$}           &   $0.013 \pm 0.013$\\
% \hline
% Bail                   & \mymodel-GCN      &   $0.768 \pm 0.044$         &       $0.695 \pm 0.042$     &  $0.815 \pm 0.029$    &  $0.024 \pm 0.013$          &    $0.039 \pm 0.018$              &  $0.022 \pm 0.011$       & $0.024 \pm 0.022$   \\
%             & \mymodel-SAGE                    &     $0.852 \pm 0.026$       &    $0.800 \pm 0.031$        &  $0.896 \pm 0.016$    &   $0.019 \pm 0.023$         &     $0.058 \pm 0.017$             & \bm{$0.003 \pm 0.002$}    &   $0.049 \pm 0.012$          \\
%             & \mymodel-infomax  &  $0.763 \pm 0.042$          &  $0.688 \pm 0.041$          &  $0.814 \pm 0.034$    &  $0.027 \pm 0.017$          &    $0.042 \pm 0.020$              &   $0.017 \pm 0.009$            & $0.024 \pm 0.022$  \\
%             & \mymodel-GIN    &  $0.825 \pm 0.019$           &  $0.769 \pm 0.019$          &   $0.872 \pm 0.013$   &    $0.017 \pm 0.015$        &      $ 0.054 \pm 0.015$            &   $0.008 \pm 0.005$            &  $0.043 \pm 0.015$ \\
%             & \mymodel-JK  &    $0.801 \pm 0.023$        &  $0.722 \pm 0.022$          &   $0.851 \pm 0.027$   &   $0.023 \pm 0.012$         & $0.043 \pm 0.020$                 &    $0.004 \pm 0.001$           & $0.032 \pm 0.018$  \\
% \hline
% Credit                   & \mymodel-GCN   &  $0.718 \pm 0.013$          &   $0.811 \pm 0.012$         &   $0.684 \pm 0.006$   &    $0.074 \pm 0.023$        &      $0.088 \pm 0.021$            &     \bm{$0.001 \pm 0.001$}          & $0.014 \pm 0.003$  \\
%             & \mymodel-SAGE           &   \bm{$0.755 \pm 0.011$}         &   \bm{$0.835 \pm 0.008$}         &   \bm{$0.740 \pm 0.008$}   &   $0.086 \pm 0.018$         & {$0.104 \pm 0.013$}       &   \bm{$0.001 \pm 0.001$}       &  \bm{$0.010 \pm 0.003$}\\
%             & \mymodel-infomax   & $0.723 \pm 0.011$           &   $0.816 \pm 0.010$         &  $0.685 \pm 0.006$    &    $0.074 \pm 0.020$        &       $0.087 \pm 0.018$           &     \bm{$0.001 \pm 0.001$}          &  $0.013 \pm 0.003$ \\
%             & \mymodel-GIN &  $0.720 \pm 0.017$          &  $0.810 \pm 0.015$          &  $0.707 \pm 0.006$    &   $0.067 \pm 0.027$         &    $0.081 \pm 0.028$              &    $0.005 \pm 0.002$           &  $0.012 \pm 0.006$  \\
%             & \mymodel-JK   & $0.745 \pm 0.016$           &  $0.812 \pm 0.026$          &  $0.688 \pm 0.015$    &   $0.057 \pm 0.022$         &  $0.079 \pm 0.020$                &   $0.002 \pm 0.001$            & $0.008 \pm 0.002$  \\
% \hline
% \end{tabular}
% \vspace{-3mm}
% \end{table*}

\begin{table*}[t]
\small
\centering
 \caption{Comparison of the performance of different variants of \mymodel.}
 \vspace{-2mm}
 \label{tab:ablation}
 \begin{tabular}{l||l||c|c|c||c|c|c|c}
 \hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{3}{c||}{Prediction Performance} & \multicolumn{4}{c}{Fairness}                     \\\cline{3-9}
                         &                         & Accuracy ($\uparrow$)   & F1-score ($\uparrow$)   & AUROC ($\uparrow$)  & $\triangle_{EO}$ ($\downarrow$) & $\triangle_{DP}$ ($\downarrow$) & $\delta_{CF}$ ($\downarrow$) & $R^2$ ($\downarrow$)\\
\hline
Synthetic                   & \mymodel-NS  &   $0.722\pm0.023$         &   $0.726\pm 0.025$         &   $0.794\pm 0.028$   &   $0.061\pm0.044$         &   $0.071\pm0.024$               &   $0.005\pm0.002$            & $0.011\pm 0.006$  \\
            & \mymodel-NN   &     $0.725 \pm 0.026$       &  \bm{$0.727 \pm 0.016$}          &    $0.794 \pm 0.024$  &   $0.066 \pm 0.048$         &  $0.086\pm0.033$                &     $0.008\pm 0.004$          &   $0.016\pm0.005$\\
            & \mymodel-NP & \bm{$ 0.729 \pm 0.022$}            &  \bm{$0.727 \pm 0.027$}          &  \bm{$0.796 \pm 0.016$}    &   $0.094 \pm 0.051$         &      $0.116 \pm 0.063$            &   $0.012 \pm 0.005$            & $0.023 \pm 0.018$  \\
            & \mymodel-NC   &   $0.720 \pm 0.019$         &   $0.725 \pm 0.018$         &  $0.793 \pm 0.018$    &   $0.058 \pm 0.042$         &    $0.069\pm 0.028$              &      $0.006 \pm 0.003$         &  $0.012 \pm 0.004$ \\
            & \mymodel  &  $0.718 \pm 0.018$          &   $0.724 \pm 0.022$         &  $0.793 \pm 0.014$    &    \bm{$0.052 \pm 0.038$}        &  \bm{$0.064 \pm 0.038$}                & \bm{$0.002 \pm 0.002$ }         &  \bm{$0.007 \pm 0.006$}     \\
\hline
Bail                   & \mymodel-NS        & $0.854 \pm 0.020$            &   $0.802 \pm 0.014$         &   $0.897 \pm 0.020$   &   $0.027\pm 0.024$         &    $0.066 \pm 0.020$              &    $0.014\pm 0.007$           & $0.056\pm 0.018$  \\
 & \mymodel-NN    &      $0.855 \pm 0.024$      &  \bm{$0.804 \pm 0.024$}          &  \bm{$0.898 \pm 0.020$}    &   $0.032 \pm 0.027$         &  $0.068\pm 0.023$                &    $0.022 \pm 0.009$           &   $0.058 \pm 0.016$\\
            & \mymodel-NP          &    \bm{$0.860 \pm 0.022$}        &    \bm{$0.804 \pm 0.031$}        &  \bm{$0.898 \pm 0.022$}    &    $0.041 \pm 0.028$        &    $0.073 \pm 0.028$           &       $0.027 \pm 0.010$           &  $ 0.064 \pm 0.019$ \\
            & \mymodel-NC       & $0.853 \pm 0.024$            &   $0.801\pm 0.019$         &  $0.896 \pm 0.021$    &     $0.025\pm 0.027$       &       $0.064\pm 0.014$           &  $0.007 \pm 0.004$             &  $0.053\pm 0.014$ \\
            & \mymodel         &     $0.852 \pm 0.026$       &    $0.800 \pm 0.031$        &  $0.896 \pm 0.016$    &   \bm{$0.019 \pm 0.023$}         &     \bm{$0.058 \pm 0.017$}             & \bm{$0.003 \pm 0.002$}    &   \bm{$0.049 \pm 0.012$}          \\
\hline
Credit                   & \mymodel-NS    & $0.749\pm 0.014$           &    $0.831\pm 0.024$        &   $0.741\pm 0.011$   &   $0.089\pm 0.018$         &      $0.109\pm 0.038$            &     $0.016\pm 0.027$          &  $0.012\pm 0.005$ \\
            & \mymodel-NN    &  $0.751\pm0.012$          &    $0.832\pm 0.018$        &    $0.742\pm 0.009$  &     $0.092\pm 0.034$       &  $0.114 \pm 0.043$                &     $0.020\pm 0.047$          & $0.013 \pm 0.004$   \\
             & \mymodel-NP  &    $0.753 \pm 0.018$        &  \bm{$0.836 \pm 0.017$}          &  \bm{ $0.749 \pm 0.010$}   &   $0.099 \pm 0.043$         & $0.122 \pm 0.049$                 &     $0.028 \pm 0.054$          & $0.016 \pm 0.007$  \\
            & \mymodel-NC    &  $0.749\pm0.015$   &  $0.830\pm0.011$          & $0.741\pm0.009$     &     $0.088\pm 0.012$       &     $0.106\pm0.011$             &  $0.004\pm 0.002$             & $0.013\pm 0.004$  \\
            & \mymodel           &   \bm{$0.755 \pm 0.011$}         &   {$0.835 \pm 0.008$}         &   {$0.740 \pm 0.008$}   &   \bm{$0.086 \pm 0.018$}         & \bm{$0.104 \pm 0.013$}       &   \bm{$0.001 \pm 0.001$}       &  \bm{$0.010 \pm 0.003$}\\
\hline
\end{tabular}
\vspace{-3mm}
\end{table*}

\vspace{-2mm}
\subsection{Experiment Settings}
\noindent\textbf{Metrics.} We evaluate the proposed framework with respect to two aspects: prediction performance and fairness. To evaluate the prediction performance, we use the widely-used node classification metrics: accuracy, F1-score, and AUROC. To measure the fairness of the representations, we first use two metrics which are commonly used in statistical fairness:
$
    \triangle_{SP} = |P(\hat{Y}_i|S_i=0)-P(\hat{Y}_i|S_i=1)|, 
$
and 
$
    \triangle_{EO} = |P(\hat{Y}_i|Y_i=1,S_i=0)-P(\hat{Y}_i|Y_i=1,S_i=1)|. 
$
% \begin{equation}
%     Unfairness = D(\mathbf{Z},\mathbf{S}),
% \end{equation}
% \begin{equation}
%     Unfairness = D(\mathbf{Z},\mathbf{S}_{N}),
% \end{equation}
To evaluate graph counterfactual fairness, we design a metric $\delta_{CF}$:
\begin{equation}
    % \delta_{CF} = |P(\hat{y}| \mathbf{S}\leftarrow \mathbf{s}')-P(\hat{y}| \mathbf{S}\leftarrow \mathbf{s}'')|,
     \delta_{CF} = |P((\hat{Y}_i)_{{S}\leftarrow \mathbf{s}'}|X=\mathbf{X},A=\mathbf{A})-P((\hat{Y}_i)_{{S}\leftarrow \mathbf{s}''}|X=\mathbf{X},A=\mathbf{A})|,
\end{equation}
% \begin{equation}
%     \delta_{CF}^n = |P(\hat{y}|s_i, S_{\neg{i}}^{(i)}\leftarrow S')-P(\hat{y}|s, S_{\neg{i}}^{(i)}\leftarrow S'')|,
% \end{equation}
%Among them, $\triangle_{SP}$ and $\triangle_{EO}$ are widely-used fairness metrics which focus on the dependency between each instance's sensitive attribute and its label.
where $\mathbf{s}',\mathbf{s}''\in \{0,1\}^n$ are arbitrary values of sensitive attribute of all nodes.
As there are too many different counterfactuals (e.g., there are $2^n$ cases for a graph with $n$ nodes), it is difficult to evaluate the difference of predictions under all these counterfactuals. Therefore, we evaluate the graph counterfactual fairness of the proposed model in the following way: on each dataset, we control the rate of sensitive subgroup population and randomly perturb the sensitive attribute of all nodes. More specifically, we randomly select $0\%, 50\%, 100\%$ nodes, and set their sensitive attribute values to be $1$, while set the sensitive attribute of other nodes to be $0$. With such perturbations, we generate counterfactual data for the whole graph with different ratios of sensitive subgroup, based on the causal model described in Section \ref{sec:dataset}. Intuitively, these perturbations implicitly control the distribution of the sensitive attribute in each node's neighborhood, and we take the averaged ratio of nodes which flip their predicted labels as an estimation for $\delta_{CF}$. Besides, we also compute the R-square $R^2(\hat{Y}_i, \tilde{{S}}_i)$ to measure how well a linear regression predictor for $\hat{Y}_i$ can be explained by the summary of the neighboring sensitive attribute values for any node $i$. Here we use the mean aggregator over the sensitive attribute values of all one-hop neighbors and each node $i$ itself to compute the sensitive attribute summary $\tilde{{S}}_i$. This R-square metric can reflect the statistical dependency between $\hat{Y}_i$ and $\tilde{{S}}_i$.

\noindent\textbf{Baselines.} We compare the proposed framework with several  state-of-the-art node representation learning methods. We divide them into two categories: 1) node representation learning methods without fairness constraints: these methods only aim to encode useful information from the input graph and improve the prediction performance in downstream tasks. We use graph convoluntional network (\textbf{GCN}) \cite{kipf2016semi}, \textbf{GraphSAGE} \cite{hamilton2017inductive}, and Graph Isomorphism Network (\textbf{GIN}) \cite{xu2018powerful} as baselines; 2) fair representation learning methods on graphs: these methods target on learning fair node representation on graphs. Among them, \textbf{C-ENC} \cite{bose2019compositional} and \textbf{FairGNN} \cite{dai2020fairgnn} enforces fairness with an adversarial discriminator to predict the sensitive attribute; \textbf{NIFTY} \cite{agarwal2021towards} enforces fairness by maximizing the similarity of representations learned from the original graph and their augmented counterfactual graphs, where the sensitive attribute values of all nodes are flipped, while other parts remain unchanged. We use two variants of it with GCN or GraphSAGE encoders, denoted by \textbf{NIFTY-GCN} and \textbf{NIFTY-SAGE}, respectively.

\noindent\textbf{Setup.} Each dataset is randomly splitted into $60\%/20\%/20\%$ training/validation/test set. Unless otherwise specified, we set the hyperparameters as $\lambda=0.6$, $C=2$, $\lambda_s=0.4$, $\beta=10$, $\mu=1e-5$, $k=20$, $B=4$. The learning rate is $0.001$, the number of epochs is $1,000$, the representation dimension is $1,024$, batch size is $100$. Experimental results are averaged over ten repeated executions. We use the Adam optimizer and implement our method with Pytorch \cite{paszke2019pytorch}.


\begin{figure}[t]
\centering
  \begin{subfigure}[b]{0.232\textwidth}
        \centering
        \includegraphics[height=1.in]{figures/encoder-pred.pdf}
        \vspace{-2mm}
        \caption{Prediction}
    \end{subfigure}
  \begin{subfigure}[b]{0.232\textwidth}
        \centering
        \includegraphics[height=1.in]{figures/encoder-fair.pdf}
        \vspace{-2mm}
        \caption{Fairness}
    \end{subfigure}
    \vspace{-2mm}
  \caption{Comparison of the performance of different subgraph encoders in GEAR on Bail dataset.}
  \label{fig:encoder}
  \vspace{-3mm}
\end{figure}

\begin{figure}[t]
\centering
  \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[height=1.in]{figures/lambda.pdf}
        \vspace{-2mm}
        \caption{$\lambda$}
    \end{subfigure}
  \begin{subfigure}[b]{0.232\textwidth}
        \centering
        \includegraphics[height=1.in]{figures/lambda_s.pdf}
        \vspace{-2mm}
        \caption{$\lambda_s$}
    \end{subfigure}
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[height=1.in]{figures/subgraph_size.pdf}
        \vspace{-2mm}
        \caption{Subgraph size $k$}
    \end{subfigure}
  \begin{subfigure}[b]{0.232\textwidth}
        \centering
        \includegraphics[height=1.in]{figures/C.pdf}
        \vspace{-2mm}
        \caption{\# of neighbor-perturbations $C$}
    \end{subfigure}
        \vspace{-2mm}
  \caption{Parameter study on Bail dataset.}
  \label{fig:parameter}
  \vspace{-3mm}
\end{figure}


\vspace{-2mm}
\subsection{Prediction Performance and Fairness}
The performance of prediction and fairness is shown in Table~\ref{tab:baseline}. The best results are shown in \textbf{bold}, and the runner-up results are \underline{underlined}. Generally speaking, we have the following observations: 
1) The proposed model \mymodel~ shows comparable prediction performance with the state-of-the-art node representation learning methods, and it outperforms all the fair node representation learning methods in prediction; 
2) The proposed model outperforms all the other fair node representation learning methods in $\delta_{CF}$ and $R^2$. 
These two fairness metrics explicitly consider the causal/statistical relation between the neighboring sensitive attribute and the model prediction, thus this observation validates the effectiveness of our framework in mitigating the biases from neighbors. 
Besides, \mymodel~ also performs well in other fairness metrics $\triangle_{EO}$ and $\triangle_{DP}$.
%
The baseline NIFTY also has good performance in graph counterfactual fairness, because NIFTY also generates counterfactuals during training. Although NIFTY does not explicitly consider the causal effect from neighbors' sensitive attribute on each node, its counterfactuals still implicitly promote graph counterfactual fairness. However, our method still outperforms all these fairness methods mainly for two reasons: a) \mymodel~ generates multiple versions of counterfactuals with self-perturbation and neighbor-perturbation. It has better coverage of the space of possible counterfactuals, while NIFTY only generates one counterfactual by flipping all nodes' sensitive attribute values, here the influence from the neighbors' sensitive attribute may counteract with each other; b) \mymodel~ generates counterfactuals which include changes in both features and graph structure after modifying the sensitive attribute, rather than simply changing the sensitive attribute. More specifically, the counterfactual augmentation component in \mymodel~ removes biases caused by misusing the descendants of the sensitive attribute in node representation learning. 

\vspace{-2mm}
\subsection{Model Structure \& Parameter Study}
To investigate the model performance under different options of model structure, we vary the encoder of subgraphs, including GCN \cite{kipf2016semi}, GraphSAGE (mean aggregator) \cite{hamilton2017inductive}, Informax \cite{velickovic2019deep}, GIN \cite{xu2018powerful}, and Jumping Knowledge (JK) \cite{xu2018representation}. %and show the model performance in Fig.~\ref{fig:encoder}. 
Due to the space limit, we only show the results in Bail in Fig.~\ref{fig:encoder}, but the observations are consistent in other datasets. Generally, all the subgraph encoders show good performance in both prediction and fairness.
% add analysis for each encoder
Among them, GraphSAGE encoder shows the best performance over all the variants.

To evaluate the robustness of \mymodel~ under different parameters, we vary the parameters $\lambda$ (the weight of constraint for graph counterfactual fairness), $\lambda_s$ (the weight for neighbor-perturbation), subgraph size $k$, and the number of neighbor-perturbations $C$ in $\mathtt{SMP}(\cdot)$ to investigate how the model performance varies. The results over different settings of parameters in Bail are shown in Fig~\ref{fig:parameter}. We observe that: 1) The model achieves better fairness with larger $\lambda$ and $\lambda_s$ while with slight sacrifice of the prediction performance; 2) The model achieves better fairness with relatively larger subgraph size, but this improvement becomes less significant when the subgraph size is over $20$. 3) When the number of neighbor-perturbations in $\mathtt{SMP}(\cdot)$ becomes larger, the predictions become more fair. These observations generally match our expectation. 

\vspace{-2mm}
\subsection{Ablation Study}
% 1. no perturbation of CF_self
% 2. no perturbation of CF_neighbors

In ablation study, we compare different variants of \mymodel~ to verify the effectiveness of different components. We first remove self-perturbations, denote this variant as \mymodel-NS. Next, we remove neighbor-perturbations, denoted by \mymodel-NN. We then remove all the perturbations, denote this variant as \mymodel-NP. We remove the counterfactual data augmentation module, just flip the sensitive attribute values, and denote this variant as \mymodel-NC. The model performance of these variants is shown in Table~\ref{tab:ablation}. We observe that all the variants perform worse than \mymodel~ with respect to fairness. These results validate the effectiveness of different components in \mymodel~ for learning fair node representations. 

% \subsection{Representation distribution}
% % summary < 0.5 vs summary > 0.5
% Aside from the prediction, we also investigate the fairness at the level of node representation. We summarize the sensitive attributes in each subgraph with mean aggregator. In Fig.~\ref{fig:representation}, we show the representation distribution in the group of nodes with $\tilde{S}<0.5$ and $\tilde{S}>0.5$ with/without perturbation. We can observe that the distribution of node representations become closer with perturbation, which validate the contribution of the perturbations in fair representation learning.

==> fmvmfnbbgqzmgyncbhqsqqzvbvfhfcxv/intro.tex <==
\section{Introduction}
% fairness on graphs
\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.235\textwidth}
        \centering
        \includegraphics[height=1.1in]{figures/gear-causal-a.pdf}
        \caption{$M'$}
    \end{subfigure}
  \begin{subfigure}[b]{0.235\textwidth}
        \centering
        \includegraphics[height=1.1in]{figures/gear-causal-b.pdf}
        \caption{$M$}
    \end{subfigure}
    \vspace{-6mm}
    \caption{Causal models generally used in existing works ($M'$) and in this work ($M$). We use $S_i,X_i, Y_i$ to denote the sensitive attribute, features, and label of any node $i$, and $A_{i,j}\in\{0,1\}$ denotes the edge between node pair $(i,j)$. Each arrow denotes a causal relation. The dashed lines denote the causal relations that the existing works do not consider.}
    \vspace{-5mm}
     \label{fig:causal}
 \end{figure}
 
Representation learning on graphs aims to map nodes into a latent embedding space. These node representations are often used to power downstream predictive tasks, and have become the new state-of-the-art in multiple real-world applications \cite{wu2020comprehensive,kipf2016semi,velivckovic2017graph,xu2018powerful}. However, these node representation learning approaches may overlook potential biases buried in the graph data, thus introducing algorithmic biases against subpopulations defined by certain sensitive attributes such as race, gender, and age. Consequently this may raise ethical and societal concerns, especially in high-stake decision-making scenarios such as {ranking of job applicants \cite{mehrabi2021survey} and credit scoring \cite{sekhon2016perceptions}}. For example, it would become a serious ethical issue if a bank's decision on the loan application was affected by the applicant's and their close contacts' race information.
 
% Recent years have witnessed a surge of research \cite{wu2020comprehensive,kipf2016semi,velivckovic2017graph,xu2018powerful} in node representation learning on graphs.
% %Recent years have witnessed a surge of research work \cite{wu2020comprehensive} in representation learning with graph data, such as graph convolutional networks (GCN) \cite{kipf2016semi}, graph attention networks \cite{velivckovic2017graph}, and Graph Isomorphism Network (GIN) \cite{xu2018powerful}.
% Despite the success of these methods in different applications, they may often introduce biases against certain subpopulations regarding sensitive attributes such as race, gender, and age. %The discrimination often occurs when the only objective of these methods is to optimize the prediction performance, thus they may overly utilize the biases in the data such as historical prejudices.
% %
% This problem has recently sparked tremendous research interests in the \textit{fairness} of node representation learning on graphs, as it is crucial to make fair decisions in many high-impact domains such as social network analysis \cite{kunegis2012fairness,fan2019graph} %, recommender systems \cite{fan2019graph}, 
% and financial services \cite{sekhon2016perceptions}. For example, in bank credit analysis, an important ethical concern is whether the banks would make decisions for loan applications based on the applicants' race.

% Existing works and limitations
To tackle the above problem, several approaches were proposed to assess and address the fairness of node representation learning on graphs. The majority of these methods aim to learn node representations which can elicit \textit{statistically} fair predictions across the population \cite{bose2019compositional,agarwal2021towards,dai2020fairgnn,li2020dyadic}. In addition, the concept of \textit{counterfactual fairness} has been extended to graph-structured data recently \cite{agarwal2021towards,agarwal2021towards2}. Different from the previous statistical notions, counterfactual fairness extends Pearl's causal structural models \cite{pearl2009causal} and aims to encourage the predictions made from different versions of the same individual (a.k.a. \textit{counterfactuals}) to be equal. For example, the prediction for one's loan application being approved should be the same regardless this applicant being Black or White.

% There have been various studies in fair node representation learning \cite{bose2019compositional,agarwal2021towards,dai2020fairgnn,li2020dyadic}, aiming to learn node representations from a given graph which can elicit fair predictions for downstream tasks. Among them, \cite{agarwal2021towards,agarwal2021towards2} extend the seminal work of \textit{counterfactual fairness} into graphs. Counterfactual fairness \cite{kusner2017counterfactual} is a fairness notion based on Pearl's causal structural models \cite{pearl2009causal}.
% %
% The intuition of counterfactual fairness is to encourage the predictions made from different versions of the same individual (a.k.a. \textit{counterfactuals}) to be equal. For example, the predictions for ``whether Jack's loan application should be approved if he had been black/white" should be the same. 
% %Existing works of counterfactual fairness on graphs \cite{agarwal2021towards} aim to minimize the discrepancy among representations learned from the original data and the counterfactuals regarding the same node. These works generate counterfactuals by changing/flipping the values of sensitive attributes of each node while keeping everything else unchanged.
% %

This paper falls under the umbrella of counterfactual fairness but focuses on addressing two critical limitations of existing studies \cite{agarwal2021towards,agarwal2021towards2} of counterfactual fairness on graphs: 1) biases induced by \textbf{one's neighboring nodes} and 2) biases induced by \textbf{the causal relations from the sensitive attributes to other features as well as the graph structure}. We follow the previous loan application example to explain these limitations in details: i) As illustrated in Fig.~\ref{fig:causal}(a), existing studies mostly focus on mitigating the causal influence from the sensitive attribute (race information $S_i$) of the $i$-th applicant on the prediction of the label (loan approval decision $Y_i$), but neglect the fact that the race information of the applicant's social contacts ($S_j$) can also causally affect the fairness of the prediction (as labeled using {\color{red} red} dashed edges in Fig.~\ref{fig:causal}(b)). 
ii) On the other hand, existing methods may implicitly assume the sensitive attribute ($S_i$) has no causal effect on other variables such as node features ($X_i$) and the graph structure ($A_{i,j}$) so that they can safely simplify the counterfactual data generation mechanism as by just flipping the sensitive attribute values. 
However, we question the applicability of this assumption since such causal effect is ubiquitous in real-world scenarios. For example, one's race %and ethnicity information 
can causally influence their social relations as well as the residential neighborhood they live in (as labeled using {\color{applegreen} green} dashed edges in Fig.~\ref{fig:causal}(b)).\footnote{There may also exist causal relations between non-sensitive features and the graph structure, although we do not show them in Fig.\ref{fig:causal} for simplicity of illustration.}
%\begin{itemize}
    % \item As illustrated in Fig.~\ref{fig:causal}(a), existing studies mostly focus on mitigating the causal influence from the sensitive attribute (race information $S_i$) of the applicant ($i$) to the prediction label (loan approval decision $Y_i$), but neglect the fact that the race information of the applicant's social contacts ($S_j$) can also causally affect the fairness of the prediction (as labeled using {\color{red} red} dashed edges in Fig~\ref{fig:causal}(b)). 
    % \item On the other hand, existing methods may implicitly assume the sensitive attribute ($S_i$) has no causal effect on other variables such as node features ($X_i$) and the graph structure ($A_{i,j}$) so that they can safely simplify the counterfactual data generation mechanism as by just flipping the sensitive attribute values. However, we question the applicability of this assumption since such causal effects are ubiquitous in real-world scenarios. For example, one's race and ethnicity information can causally influence their social relations as well as the residential neighborhood they choose to live in (as labeled using {\color{applegreen} green} dashed edges in Fig~\ref{fig:causal}(b)).
%\end{itemize}

% However, most existing work of counterfactual fairness on graphs \cite{agarwal2021towards,agarwal2021towards2} are based on some unrealistic assumptions about the causal model, which lead to limitations in their methods. Fig.~\ref{fig:causal}(a) shows a commonly used causal model in many existing works, and we use a toy example of loan application to intuitively explain these limitations.
% Here we aim to predict whether the loan application can be approved ($Y_i$) for each applicant $i$ with sensitive attribute $S_i$ and other features $X_i$, and we have the social relations $A_{i,j}$ between $i$ and any other individual $j$. Most existing works have the following limitations:
% 1) \textbf{Biases from neighboring effect:} These works are overwhelmingly devoted to eliminating the causal influence of the sensitive attribute of a node to its own predicted label by regularizing node representation, but neglect the fact that for a node, the sensitive attributes of some other relevant nodes (e.g., neighbors) may also causally affect this node's label, and lead to unfair predictions. 
% %Most existing works are overwhelmingly devoted to eliminating the influence of the sensitive attribute of each node to its corresponding prediction by regularizing node representation, but neglect the fact that for each node, the sensitive attributes of some other relevant nodes (e.g., neighbors) may also causally affect this node's prediction label, and lead to unfair predictions. 
% %
% For example, recent studies \cite{li2020fairness} have shown that, decision makers often utilize the applicants’ neighbors in social network for real-world credit evaluation and approval. In such scenarios, the label of a node can be causally affected by its neighbors' sensitive attributes (such causal relations are shown as the red dashed directed edges in Fig~\ref{fig:causal}(b)). Existing methods which ignore such causal relations 
% can explicitly or implicitly utilize the neighbors' sensitive attributes in the training process to minimize the training loss, and thus result in unfair predictions. 
% %, e.g., an applicant who have many friends of a certain sensitive subgroup may bring unfair biases to this applicant's application. This observation results from direct or indirect causal associations from the sensitive attributes of each node' neighbors to its label. 
% %In this case, such biases in the labels will be utilized in the training process of machine learning models, thus leading to representations that would result in unfair predictions; 
% 2) \textbf{Biases in features and graph:} Most existing methods  \cite{agarwal2021towards,agarwal2021towards2} are based on na\"ive counterfactual data generation mechanisms, i.e., just flipping the sensitive attribute values of all nodes. Such mechanisms are based on the implicit assumption that the sensitive attribute has no causal effect on other variables such as node features and the graph structure.
% %
% However, in real-world scenarios, such causal effects are ubiquitous. For example, the social relationship and many covariates (e.g., home address) of an individual would likely be different if her/his race had been changed, as the causal relations shown as green dashed directed edges in Fig.~\ref{fig:causal}(b). 
% %
% In these cases, the biased features and graph structures resulting from such causal effects may also be misused by machine learning models, which further leads to unfair predictions.

%However, most of these existing works are overwhelmingly devoted to eliminating the dependency between the sensitive attributes of each node and the corresponding prediction based on the learned representation, but neglect a fact that the sensitive attributes of the node's neighbors may also be utilized in the graph representation learning models, and thus lead to discrimination in the learned representation. 

    % three kinds of dependency between S_N(i) and Y_i
%This observation may results from various kinds of associations between neighbors’ sensitive attributes and the labels: 1) some sensitive attributes such as obesity [] may be contagious to neighbors, i.e., affect the neighbors to have similar attributes, thus the neighbors' sensitive attributes may indirectly affect the labels; 2) the neighbors' sensitive attributes may 

We argue that biases in model predictions can be induced by the aforementioned pathways.  %therefore unfair predictions can still be made from machine learning algorithms.
In this paper, we propose a more comprehensive fairness notion on graphs -- \textit{graph counterfactual fairness}, %which considers the potential biases brought by the causal influence from the sensitive attributes of a node and its relevant nodes (e.g., neighbors) on other variables (labels, features and graph structure) of the node. 
which considers the potential biases regarding the sensitive attributes of each node and its neighboring nodes, as well as the biases led by the causal effect  from sensitive attributes on other variables. %of the node.
% not only the causal relation from each node's sensitive attribute to the prediction label of the corresponding node, but also the causal effect of the sensitive attribute of the neighboring nodes on the prediction label.
%
%Furthermore, we also take considerations of the biases embedded in features and graph structure due to the causal effect from the sensitive attributes of each node and their neighbors. 
%
With this notion, learning node representations towards graph counterfactual fairness is still challenging. It is because the causal relations among  variables (as showed in Fig.~\ref{fig:causal}(b)) are often required to obtain the counterfactuals, but these causal relations are often unknown in practice. 
Manually constructing the entire causal model requires extensive domain knowledge and human efforts, %as well as incredible amount of human efforts, 
especially for large-scale graph data.
% More specifically, we aim to mitigate the above biases and learn representations which can achieve graph counterfactual fairness.
% % challenge: 1) S_N(i) -> y 2) counterfactual 3) counterfactual + neighbor 
% This problem remains a daunting task due to the following challenges: 
% 1) The ground-truth causal model w.r.t. variables of all the nodes in a graph is often unknown. The biases led by the causal effect from other nodes' sensitive attributes on the labels might be difficult to model and eliminate, especially when the graph is large-scale; 
% 2) Due to the lack of ground-truth causal models, we do not have enough prior knowledge to describe the causal relationships among different variables (even in independent and identically distributed data), e.g., sensitive attributes, the other nodes' features, the graph structure, and the label. Therefore, it can be extremely challenging to generate counterfactuals. 
%3) If consider the graph structure, the variables of different nodes may influence each other, so the causal model can be even more complicated, especially when the whole graph is sizable. This scenario makes it even harder to mitigate the influence of the sensitive attribute of other nodes on the prediction target, as well as generate counterfactuals for the neighbors' sensitive attribute values. 
%1) how to formulate the new fairness notion on graphs; 2) how to eliminate the causal effect of selfs' and neighbors' sensitive attributes on the labels; 3) how to evaluate the graph counterfactual fairness.
% 1. Siamese network + counterfactual data augmentation 2. counterfactual data 3. subgraph
To address the above challenge, we propose a novel framework to learn \textbf{G}raph count\textbf{E}rfactually f\textbf{A}ir node \textbf{R}epresentations (\textbf{\mymodel}). \mymodel~ aims to learn node  representations towards graph counterfactual fairness, and maintain high performance for downstream tasks such as node classification.
\mymodel~ includes the following modules: 
%\begin{itemize}
    1) \textbf{Subgraph generation.} %To reduce computation costs on large graphs, 
    {To reduce the costs of modeling the causal relations on large graphs, }
    we first develop an algorithm to automatically infer the importance scores among nodes. For each individual node, we then prune the range of the causal model to an ego-centric subgraph which contains only the node itself and its most influential neighboring nodes. 
    2) \textbf{Counterfactual data augmentation.} For each node, we leverage the graph auto-encoder technique \cite{kipf2016variational} and fairness constraints to generate two types of counterfactuals as data augmentation: 1) self-perturbation: the counterfactuals where each node's own sensitive attribute value had been modified; 2) neighbor-perturbation: the counterfactuals where the sensitive attribute values of neighbors had been modified.
    3) \textbf{Node representation learning.} To learn node representations towards graph counterfactual fairness, %mitigate the impact from a node's and its neighbors' sensitive attributes on the node representation, 
    we leverage a Siamese network \cite{bromley1993signature} to minimize the discrepancy between the representations learned from the original subgraph and those learned from counterfactuals.
%\end{itemize}
%
%Specifically, based on a common assumption \cite{jiao2020sub}, the graph nodes are mostly influenced by its regional nearest neighbors. %
% In this framework, to avoid the over-sizing problem in graphs, we take each node as a central node, and generate a subgraph which contains this central node and its nearest neighbors with the highest important scores. These important scores measure the ``proximity" between different nodes to the central node. This is based on a commonly used assumption that, in a graph, a node is mostly influenced by its regional nearest neighbors. We use these subgraphs to approximately and more feasibly capture the causal impact from other nodes. %, and improve the feasibility of modeling the causal relations on graph. %and can remarkably reduce the load of modeling the causal relations among all the nodes in the whole graph.
% %
% To mitigate the impact from a node's and its neighbors' sensitive attributes on its representation, \mymodel~ leverages a Siamese network \cite{bromley1993signature} to minimize the discrepancy between the representations learned from the original subgraph and those learned from counterfactuals. For each node, we generate two types of counterfactuals as data augmentation: 1) self-perturbation: the counterfactual where each node's own sensitive attribute had been modified; 2) neighbor-perturbation: the counterfactuals where the sensitive attributes of neighbors had been modified. Features and graph structure can also be changed according to these perturbations.
% %
% To generate the counterfactuals, we develop a counterfactual data augmentation module, which is based on some simple but general assumptions of the causal model, using graph auto-encoder \cite{kipf2016variational} and fairness constraints to capture the latent factors which are not causally influenced by the sensitive attribute of any node. Then we generate counterfactuals with these captured factors and any sensitive attribute values assigned to all the nodes.
%
%Besides, an additional advantage of such subgraphs is that the subgraphs are separate with each other, so we can generate any counterfactuals for each node's corresponding subgraph without any conflict, which makes the whole model training process more flexible and disentangled.
The main contributions of this work can be summarized as follows:
\begin{itemize}
\item \textbf{Problem.} We propose a new fairness notion --- graph counterfactual fairness, which considers the potential biases brought by different causal pathways from sensitive attributes to the graph model predictions.
%
%We present a formal definition of this fairness notion, discuss its connection and distinction with other notions, and analyze the importance and challenges of graph representation learning regarding this fairness notion.
\item \textbf{Method.} We propose a novel framework \mymodel~ to learn node representations towards graph counterfactual fairness. Specifically, for each node, we minimize the discrepancy between the representations learned from the original data and the augmented counterfactuals with different sensitive attribute values.
\item \textbf{Experiments.} We conduct extensive experiments on both synthetic and real-world graphs.
%
The results show that the proposed method outperforms existing baselines in multiple fairness notions, and achieves comparable prediction performance in downstream tasks.
\end{itemize}

==> fmvmfnbbgqzmgyncbhqsqqzvbvfhfcxv/macros.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{question}[theorem]{Question}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{example}[theorem]{Example}
\newtheorem{thm}[theorem]{Theorem}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{lem}[theorem]{Lemma}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{note}[theorem]{Note}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{conjecture*}{Conjecture}
\newtheoremstyle{nonindented}{1ex}{1ex}{}{}{\bfseries}{.}{.5em}{}
\newtheoremstyle{indented}{1ex}{1ex}{\itshape\addtolength{\leftskip}{0.6cm}\addtolength{\rightskip}{0.6cm}}{}{\bfseries}{.}{.5em}{}
\theoremstyle{nonindented}
%\newtheorem{domain}{Game Domain}
\theoremstyle{indented}
%\newtheorem{question}{Question}[section]
%\newtheorem*{direction*}{Research Direction}
%\newtheorem*{conjecture*}{Conjecture}
\theoremstyle{plain}



\newenvironment{proofof}[1]{\begin{proof}[Proof of #1]}{\end{proof}}
\newenvironment{proofsketch}{\begin{proof}[Proof Sketch]}{\end{proof}}
\newenvironment{proofsketchof}[1]{\begin{proof}[Proof Sketch of #1]}{\end{proof}}

\newenvironment{alg}{\begin{algorithm}\begin{onehalfspace}\begin{algorithmic}[1]}{\end{algorithmic}\end{onehalfspace}\end{algorithm}} 

\newcommand{\mult}{\times}
\newcommand{\cross}{\times}
\newcommand{\by}{\times}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\bvec}[1]{\boldsymbol{ #1 }}
\newcommand{\card}[1]{\left| #1 \right|}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}
\newcommand{\bigunion}{\bigcup}
\newcommand{\bigintersect}{\bigcap}
\newcommand{\sm}{\setminus}
\newcommand{\floor}[1]{\lfloor {#1} \rfloor}
\newcommand{\ceil}[1]{\lceil {#1} \rceil}
\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\bar}{\overline}
\newcommand{\iid}{i.i.d.\ }

\newcommand{\lt}{\left}
\newcommand{\rt}{\right}


\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\polylog}{polylog}

%Operators: These operators are such that a subscript appears below
%in \[ \] math mode, and to the bottom right in regular $ $ math mode

%regular version
\def\pr{\qopname\relax n{Pr}}
\def\ex{\qopname\relax n{E}}
\def\min{\qopname\relax n{min}}
\def\max{\qopname\relax n{max}}
\def\argmin{\qopname\relax n{argmin}}
\def\argmax{\qopname\relax n{argmax}}
\def\avg{\qopname\relax n{avg}}


%bold version
\def\Pr{\qopname\relax n{\mathbf{Pr}}}
\def\Ex{\qopname\relax n{\mathbf{E}}}
\def\supp{\qopname\relax n{\mathbf{supp}}}
\def\Min{\qopname\relax n{\mathbf{min}}}
\def\Max{\qopname\relax n{\mathbf{max}}}
\def\Argmin{\qopname\relax n{\mathbf{argmin}}}
\def\Argmax{\qopname\relax n{\mathbf{argmax}}}
\def\Avg{\qopname\relax n{\mathbf{avg}}}
\def\vol{\qopname\relax n{\mathbf{vol}}}
\def\aff{\qopname\relax n{\mathbf{aff}}}
\def\conv{\qopname\relax n{\mathbf{convexhull}}}
\def\hull{\qopname\relax n{\mathbf{hull}}}

\newcommand{\expect}[2][]{\ex_{#1} [#2]}

\newcommand{\RR}{\mathbb{R}}
\newcommand{\RRp}{\RR_+}
\newcommand{\RRpp}{\RR_{++}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\QQ}{\mathbb{Q}}

\def\A{\mathcal{A}}
\def\B{\mathcal{B}}
\def\C{\mathcal{C}}
\def\D{\mathcal{D}}
\def\E{\mathcal{E}}
\def\F{\mathcal{F}}
\def\G{\mathcal{G}}
\def\H{\mathcal{H}}
\def\I{\mathcal{I}}
\def\J{\mathcal{J}}
\def\K{\mathcal{K}}
\def\L{\mathcal{L}}
\def\M{\mathcal{M}}
\def\P{\mathcal{P}}
\def\R{\mathcal{R}}
\def\S{\mathcal{S}}
\def\O{\mathcal{O}}
\def\T{\mathcal{T}}
\def\V{\mathcal{V}}
\def\X{\mathcal{X}}
\def\Y{\mathcal{Y}}

\def\eps{\epsilon}
\def\sse{\subseteq}

\def\SS{\mathbb{S}}

\newcommand{\pmat}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\Bmat}[1]{\begin{Bmatrix} #1 \end{Bmatrix}}
\newcommand{\vmat}[1]{\begin{vmatrix} #1 \end{vmatrix}}
\newcommand{\Vmat}[1]{\begin{Vmatrix} #1 \end{Vmatrix}}
\newcommand{\mat}[1]{\pmat{#1}}
\newcommand{\grad}{\bigtriangledown}
\newcommand{\one}{{\bf 1}}
\newcommand{\zero}{{\bf 0}}


\newcommand{\eat}[1]{}


\newcommand{\hl}[1]{{\bf \color{red}#1}}
\newcommand{\todo}[1]{{\hl{To do: #1}}}
\newcommand{\change}[1]{{\hl{#1}}}
\newcommand{\todof}[1]{{\hl{ (Todo\footnote{\hl{\bf  To do: #1}})}}  }
\newcommand{\noi}{\noindent}
\newcommand{\prob}[1]{\vspace{.2in} \noindent {\bf Problem #1.}\\}
\newcommand{\subprob}[1]{ \vspace{.2in} \noindent {\bf #1.}\\}


%Plain eps or pdf figure. Use IPE to embed tex in it.
\newcommand{\fig}[2][1.0]{
  \begin{center}
    \includegraphics[scale=#1]{#2}
  \end{center}}
%Combined PS/Latex figure. This is option of choice for including tex
%code from xfig. Remember to export from xfig using "combined ps/latex" option
\newcommand{\figpst}[2][0.8]{
  \begin{center}
    \resizebox{#1\textwidth}{!}{\input{#2.pstex_t}}
  \end{center}}
%Combined PDF/Latex figure. This is option of choice for including tex
%code from xfig. Remember to export from xfig using "combined pdf/latex" option
\newcommand{\figpdft}[2][0.8]{
  \begin{center}
    \resizebox{#1\textwidth}{!}{\input{#2.pdf_t}}
  \end{center}}



%Algorithmic Environment stuff
\newcommand{\INPUT}{\item[\textbf{Input:}]}
\newcommand{\OUTPUT}{\item[\textbf{Output:}]}
\newcommand{\PARAMETER}{\item[\textbf{Parameter:}]}


%LP environment stuff
\newcommand{\mini}[1]{\mbox{minimize} & {#1} &\\}
\newcommand{\maxi}[1]{\mbox{maximize} & {#1 } & \\}
\newcommand{\maxis}[1]{\mbox{max} & {#1 } & \\}
\newcommand{\minis}[1]{\mbox{min} & {#1 } & \\}
\newcommand{\find}[1]{\mbox{find} & {#1 } & \\}
\newcommand{\st}{\mbox{subject to} }
\newcommand{\sts}{\mbox{s.t.} }
\newcommand{\con}[1]{&#1 & \\}
\newcommand{\qcon}[2]{&#1, & \mbox{for } #2.  \\}
\newenvironment{lp}{\begin{equation}  \begin{array}{lll}}{\end{array}\end{equation} }
\newenvironment{lp*}{\begin{equation*}  \begin{array}{lll}}{\end{array}\end{equation*}}



\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
%% MISC





==> fmvmfnbbgqzmgyncbhqsqqzvbvfhfcxv/method.tex <==
\section{The Proposed Framework --- GEAR}
\begin{figure*}[t]
\centering
     \includegraphics[width=.82\textwidth,height=2.8in]{figures/fm_cropped.pdf}
     \vspace{-0.15in}
      \caption{An illustration of the proposed framework \mymodel.}
      \vspace{-0.1in}
       \label{fig:model_1}
\end{figure*}

In this section, we propose a novel framework \mymodel~ which aims to learn node representations for graph counterfactual fairness. As the illustration shown in Fig.~\ref{fig:model_1}, \mymodel~ mainly includes three key components: 1) subgraph generation; 2) counterfactual data augmentation; 3) fair representation learning. In subgraph generation, \mymodel~ extracts a context subgraph for each node, which contains the local graph structure including the node itself (central node) and its nearest neighbors with respect to precomputed importance scores.
%
In counterfactual data augmentation, we generate counterfactuals in which the sensitive attribute of nodes in these subgraphs had been perturbed. % self- and neighbor- perturbation?
%the proposed framework leverages the augmented counterfactual data to learn fair representations.
%
Based on the augmented counterfactuals, the fair representation learning component leverages Siamese networks \cite{bromley1993signature} to minimize the distance between the representations learned from the original data and the counterfactuals w.r.t. the same node. 

%fairness notion, and leverage  counterfactual data augmentation to learn fair representations. The proposed framework mainly includes two key components: 1) subgraph generation; 2) counterfactual data augmentation; 3) fair representation learning. In subgraph based counterfactual data augmentation, we sample a context subgraph for each node, and generate two kinds of counterfactuals of this subgraph based on perturbation of the sensitive attributes in the subgraph; and in the fair representation learning component, we use Siamese networks \cite{bromley1993signature} to minimize the distance between the representation learned from the original subgraph and the counterfactual subgraphs. 

%\subsection{Subgraph based counterfactual data augmentation }
\vspace{-2mm}
\subsection{Subgraph Generation}
True causal models for graph data are often difficult to be completely obtained, %thus the causal effect from the sensitive attribute of other nodes in the graph on the labels, as well as the causal relations among different variables can be complicated, 
especially for large-scale graphs.
% 
Based on a common observation \cite{hamilton2017inductive,jiao2020sub} that each node is mostly influenced by its nearest neighbors, we extract a subgraph $\mathcal{G}^{(i)}$ with node features $\mathbf{X}^{(i)}$ and adjacency matrix $\mathbf{A}^{(i)}$ for each node $i$.
% %
This subgraph extracts the context information of the central node $i$ on $\mathcal{G}$, i.e., the subgraph of $\mathcal{G}$ which only contains the top $k$ neighbors of node $i$ (including itself). These top-$k$ neighbors are usually within several hops from the central node. 
%We assume that the nodes outside the subgraph $\mathcal{G}^{(i)}$ is independent with the features, graph structure and the label/predicted label of node $i$. 
%
Specifically, for each node $i$ on the graph, we generate its context subgraph $\mathcal{G}^{(i)}$ with a subgraph generator $\mathtt{Sub}(\cdot)$. % By intuition, once we select a central node, its nearest neighbors and the local graph structure form the subgraph.
%
Based on these context subgraphs, we learn the representations for their corresponding central nodes. This is based on a commonly used assumption \cite{hamilton2017inductive} that each node has a low dependency with the nodes outside its context subgraph. Therefore, each subgraph is expected to be informative enough with respect to the graph structure relative to the central node for high-quality representation learning and counterfactual data augmentation afterwards.
%

%In the subgraph generator, 
Inspired by recent subgraph based node representation learning methods \cite{jiao2020sub,zhang2020graph}, we first compute the importance scores for every node pair with personalized pagerank algorithm \cite{jeh2003scaling}. The importance scores can be calculated as:
$
\mathbf{R}= \alpha (\mathbf{I}-(1-\alpha)\bar{\mathbf{A}}),
$
where $\mathbf{R}$ is the importance score matrix, and each entry $\mathbf{R}_{i,j}$ describes how important node $j$ is for node $i$, and $\mathbf{R}_{i,:}$ denotes the importance score vector for node $i$.
%
$\alpha$ is a parameter in the range of $[0,1]$, $\mathbf{I}$ is the identity matrix. $\bar{\mathbf{A}}=\mathbf{A}\mathbf{D}^{-1}$ denotes the column-normalized adjacency matrix, where $\mathbf{D}$ is the corresponding diagonal matrix with $\mathbf{D}_{i,i}=\sum_j{\mathbf{A}_{i,j}}$.
%
We compute $\mathbf{R}$ in a preprocessing stage before model training for efficiency.
%The score can be calculated with different metrics []. A simple implementation is to use the distance between a pair of nodes to compute the score, e.g., $r(j,i)=1/d(j,i)$, where $d(j,i)$ is the distance (length of the shortest path) from $j$ to $i$. This is based on the commonly used assumption that nodes with closer distance tend to have strong influence to each other. 
With the importance scores, we use a $\mathtt{TOP(\cdot)}$ operation to select the top-$k$ important nodes $\mathcal{V}^{(i)}$ for each central node $i$, then formulate the context subgraph $\mathcal{G}^{(i)}$ as follows:
\begin{equation}
    \mathcal{G}^{(i)} = \{\mathcal{V}^{(i)},\mathcal{E}^{(i)}, \mathbf{X}^{(i)}\} = \{\mathbf{A}^{(i)}, \mathbf{X}^{(i)}\},
    \label{eq:subgraph_gen}
\end{equation}
\begin{equation}
 \mathcal{V}^{(i)} = \mathtt{TOP}(\mathbf{R}_{i,:}, k),
\end{equation}
\begin{equation}
 \mathbf{A}^{(i)} = \mathbf{A}_{\mathcal{V}^{(i)}, \mathcal{V}^{(i)}}, \,\,\mathbf{X}^{(i)} = \mathbf{X}_{\mathcal{V}^{(i)},:},
 \label{eq:subgraph_gen_feature}
\end{equation}
% \begin{equation}
%  \mathbf{X}^{(i)} = \mathbf{X}_{\mathcal{V}^{(i)},:},
%  \label{eq:subgraph_gen_feature}
% \end{equation}
where the symbol $:$ means all the indices. The above subgraph generation process (Eq.~\eqref{eq:subgraph_gen} to~\eqref{eq:subgraph_gen_feature}) is defined as $\mathcal{G}^{(i)}=\mathtt{Sub}(i, \mathcal{G}, k)$. Then the generated subgraphs are fed into encoders to learn representations of the central nodes.

\subsection{Counterfactual Data Augmentation} 
\label{subsec:cf_da}
To achieve graph counterfactual fairness, we pretrain a counterfactual data augmentation module before node representation learning.
%We first select a set of nodes $\mathcal{V}^c$ from $\mathcal{V}$, and generate counterfactual data by perturbing their context subgraphs in the following steps. A straightforward way of node selection is to select all the nodes in the graph, i.e., $\mathcal{V}^c=\mathcal{V}$, but it might be too expensive for large-scale graphs, so we can also select those nodes which are more important in the graph, or more possible to suffer from discrimination led by the network. A typical choice is the nodes which have larger degree may be under stronger influence from others. Another choice is the individuals whose neighboring nodes have the same or similar sensitive attributes, for example, those people in a community which only consists of a certain race of people may tend to suffer from more biases. 
%In order to quantify these selection criterion
%Based on Pearl's structural causal model \cite{pearl2009causal}, the ground-truth counterfactuals should be generated based on a given causal model. However, such causal model is often very difficult to be precisely obtained for real-world datasets, even on i.i.d. data. 
Here we consider a relatively simple but general causal model (as shown in Fig.~\ref{fig:causal}(b)) to generate counterfactuals for each subgraph. 
%
Based on common observations \cite{kusner2017counterfactual}, we assume that the sensitive attribute (e.g., race) is exogenous, i.e., it has no parent variables in the causal graph, and it would causally influence the other node features, the graph structure, and the labels. 
Based on the causal model we assume, once we intervene on the sensitive attribute, we need to model how the other variables change accordingly. To achieve this goal, we use a graph variational auto-encoder (GraphVAE) \cite{kipf2016variational} based module, which takes each context subgraph as input and encodes each node in the subgraph into a latent embedding $\mathbf{h}_i$, then a decoder reconstructs the original subgraph with the latent embeddings $\mathbf{H}=\{\mathbf{h}_1,...,\mathbf{h}_k\}$ and the sensitive attribute values of the $k$ nodes in this subgraph. The reconstruction loss $\mathcal{L}_r$ is as follows (we leave out the superscript $(\cdot)^{(i)}$ for notation simplicity):
\begin{equation}
    \mathcal{L}_r = \mathbb{E}_{q({H}|\mathbf{X},\mathbf{A})}[-\log(p(\mathbf{X},\mathbf{A}|H, \mathbf{S}))] + \text{KL}[q({H}|\mathbf{X},\mathbf{A})\|p({H})],
\end{equation}
% \begin{equation}
% \label{eq:loss_cf}
%     \mathcal{L}_a = \mathbb{E}_i[\mathcal{L}_r(i)] + \beta \text{MI}(\mathbf{H}, \tilde{\mathbf{S}}),
% \end{equation}
% \begin{equation}
%     \mathcal{L}_r(i) = l(G(\mathbf{H}^{(i)}), \mathcal{G}^{(i)}),
% \end{equation}
where %$\mathcal{L}_r$ is the reconstruction loss on each subgraph $\mathcal{G}^{(i)}$, 
$p({H})$ is a standard Normal prior distribution. We sample the embeddings $\mathbf{H}$ from $q({H}|\mathbf{X},\mathbf{A})$. 
%$\mathbf{H}$ denotes the representation for any random node, 

As the sensitive attribute is assumed to be exogenous, we can mitigate the causal effect from the sensitive attribute on the embeddings by removing the statistical dependency between them. To achieve this target, we use an adversarial learning method to learn embeddings which are invariant to different sensitive attribute values of each node and their neighbors. Specifically, we use a discriminator here to predict the summary of neighboring sensitive attribute values. Here we take the summary $\tilde{s}_i$ as the mean aggregation over all the nodes in the subgraph $\mathcal{G}^{(i)}$, i.e., $\tilde{s}_i=\frac{1}{|\mathcal{V}^{(i)}|}\sum_{j\in \mathcal{V}^{(i)}}s_j$. We divide the summary into $B$ ranges to formulate it as a multivariate classification task for the discriminator $D(\cdot)$. We use a fairness constraint as follows:
%\vspace{-1mm}
$%\begin{equation}
    \mathcal{L}_d = \sum\nolimits_{b\in [B]}\mathbb{E}[\log(D(\mathbf{H}, b))],
%    \vspace{-1mm}
$%\end{equation}
where the discriminator $D(\mathbf{H}, b)$ predicts the probability of whether the summary of sensitive attribute values is in range $b$. Based on the theoretic analysis in \cite{song2020novel,bose2019compositional}, $\mathcal{L}_d$ is a regularizer to minimize the mutual information between the summary of sensitive attribute values and the embeddings. The final loss of the counterfactual data augmentation is:
$
    \mathcal{L}_a = \mathcal{L}_r + \beta \mathcal{L}_d,
$
where $\beta$ is a hyperparameter for the weight of fairness constraint. We use alternating stochastic gradient descent for optimization: 1) we minimize $\mathcal{L}_a$ by fixing the discriminator and updating parameters in other parts; 2) we minimize $-\mathcal{L}_a$ with respect to the discriminator while other parts fixed.
%$\tilde{\mathbf{S}}$ denotes an aggregation of sensitive attribute values over the neighbors. Here, we use the mean aggregator. The second term in Eq.~\ref{eq:loss_cf} aims to minimize the mutual information between the sensitive attribute aggregated in the neighborhood and the latent representation. We then use $G(\cdot)$ to reconstruct the original graph based on the learned representation.
%
To achieve graph counterfactual fairness, we expect the embeddings  $\mathbf{H}$ can capture the latent variables %in the simple causal model
which are informative of the input subgraph but not causally influenced by the sensitive attribute of the nodes in the subgraph.
%As the sensitive attribute has no parent variables, we can remove the 
%and calculated in three steps: %1) Abduction: compute the values of the set of unobserved variables given the causal model; 2) Action: Replace the  sensitive attribute variable with a specific value w in the model equations; 3. Prediction: Using the new model equations, and U (or P(U |X )) compute the value of V (or P (V |X )).
We pretrain the counterfactual data augmentation module to better disentangle different components of the framework. If more prior knowledge of the causal model is provided, we can incorporate it in counterfactual data augmentation, e.g., directly generate counterfactuals with a given causal model, and do not need to change other components in the framework.

Based on the above techniques, we conduct perturbations on the original subgraphs and obtain different types of counterfactuals. For each context subgraph $\mathcal{G}^{(i)}$, we generate two kinds of perturbations on it, including self-perturbation on the sensitive attribute of the central node, and neighbor-perturbation on the sensitive attribute of other nodes in the subgraph.

\noindent\textbf{Self-perturbation.} In the subgraph $\mathcal{G}^{(i)}$, we take its node embeddings, flip the sensitive attribute value of the central node ${s}_i$, then feed the embeddings and the perturbed sensitive attribute into the decoder of the pretrained counterfactual data augmentation module, and take the reconstructed subgraph as the corresponding counterfactual.
%For sensitive attributes which are categorical variables with $m$ values, we sample a different value from the original one with $1/(m-1)$ probability. For continuous sensitive attributes, we uniformly sample from the space of the variable. 
The set containing the subgraphs after self-perturbation is denoted by $\mathcal{\bar{G}}^{(i)}=\{\mathcal{G}^{(i)}_{{S}_i\leftarrow {1-s_i}}$\}. %, where $|\mathcal{\bar{G}}^{(i)}|=1$. 
%where the operation $\mathtt{SMP(\cdot)}$ uniformly samples a specific value of the sensitive attribute out of the value space $\mathcal{S}$, which is different from the original value $\mathbf{s}_i$.

\noindent\textbf{Neighbor-perturbation.} Similarly, in the subgraph $\mathcal{G}^{(i)}$, we randomly perturb the sensitive attribute values of any nodes except the central node, i.e., the nodes in the set $\mathcal{V}^{(i)}_{\neg i}$. After such perturbation, we generate a set of counterfactuals $\mathcal{\underline{G}}^{(i)}=\{\mathcal{G}^{(i)}_{{S}^{(i)}_{\neg i}\leftarrow{\mathtt{SMP}({\mathbf{S}^{(i)}_{\neg i}})}}\}$, where $\mathtt{SMP}(\cdot)$ randomly samples specific values of the sensitive attribute out of the value space $\{0,1\}^{|\mathcal{V}^{(i)}|-1}$. %and they are different from the original values $\mathbf{S}^{(i)}_{\neg i}$. % We propose two strategies of perturbation here:
% \begin{itemize}
%     \item \textbf{Random perturbation.} All the nodes in $\mathcal{V}^{(i)}_{\neg i}$ have the same probability to be perturbed, i.e., for each node $j\in\mathcal{V}^{(i)}_{\neg i}$, we use $\mathtt(\cdot)$ to sample a different value from the original one.
%     \item \textbf{Weighting.} As the infl
% \end{itemize}
%As the above perturbation consists of sampling, 
We use a parameter $C$ to denote the number of  $\mathtt{SMP}(\cdot)$ operations in neighbor-perturbation.
%the number of counterfactual subgraphs sampled from neighbor-perturbation. %i.e., $|\mathcal{\underline{G}}^{(i)}|=C$. 
%For each node $i$, we denote the sets of these two kinds of counterfactual subgraphs as $\{\mathcal{\bar{G}}^{(i)}\}$ and $\{\mathcal{\underline{G}}^{(i)}\}$, respectively, where $|\mathcal{\underline{G}}^{(i)}|=C$.

%In this framework, we design  the counterfactual data augmentation and fair representation learning because we

\vspace{-2mm}
\subsection{Fair Representation Learning}
%
Based on the above counterfactual data augmentation, we learn fair representations which are expected to elicit the same predicted label across different counterfactuals w.r.t. the same node. 
To achieve this goal, we leverage Siamese networks \cite{bromley1993signature} to encode the three kinds of subgraphs: original subgraphs $\mathcal{G}^{(i)}$, counterfactual subgraphs $\mathcal{\bar{G}}^{(i)}$ and $\mathcal{\underline{G}}^{(i)}$ for each central node $i$. For graph counterfactual fairness, we expect to learn the same representations for each central node from the three kinds of subgraphs. 
We train a subgraph encoder $\phi(\cdot)$ to generate the representations $\mathbf{z}_i$, $\mathbf{\bar{z}}_i$, $\mathbf{\underline{z}}_i$ for each central node $i$ on these three kinds of subgraphs, respectively. Then we  minimize the distance between the central node representations learned from the original subgraph and from the counterfactuals. We formulate the loss for graph counterfactual fairness as:
\begin{equation}
    \mathcal{L}_f = \frac{1}{|\mathcal{V}|}\sum\nolimits_{i\in \mathcal{V}}((1-\lambda_s) d(\mathbf{z}_i, \mathbf{\bar{z}}_i) + \lambda_s d(\mathbf{z}_i, \mathbf{\underline{z}}_i)),
\end{equation}
where $d(\cdot)$ is a distance metric such as cosine distance. $\lambda_s\in [0,1]$ is a hyperparameter which controls the weight of neighbor-perturbation. From the original subgraph and the counterfactuals, we obtain the node representations in the following way: 
\begin{equation}
    \mathbf{z}_i %= \phi(\mathcal{G}^{(i)})_i
    =(\phi(\mathbf{X}^{(i)}, \mathbf{A}^{(i)}))_i,
\end{equation}
\begin{equation}
    \mathbf{\bar{z}}_i  %=\mathtt{AGG}(\{\phi(\mathcal{\bar{G}}^{(i)})_i\})
    =\mathtt{AGG}(\{(\phi(\mathbf{X}_{{S}_i\leftarrow{1-s_i}}^{(i)}, \mathbf{A}_{S_i\leftarrow{1-s_i}}^{(i)}))_i\}),
\end{equation}
\begin{equation}
    \mathbf{\underline{z}}_i = %\mathtt{AGG}(\{\phi(\mathcal{\underline{G}}^{(i)})_i\}) =
    \mathtt{AGG}(\{(\phi(\mathbf{X}_{{S}^{(i)}_{\neg i}\leftarrow\mathtt{SMP}(\mathbf{S}^{(i)}_{\neg i})}^{(i)}, \mathbf{A}^{(i)}_{{S}^{(i)}_{\neg i}\leftarrow\mathtt{SMP}(\mathbf{S}^{(i)}_{\neg i})}))_i\}),
\end{equation}
where $\phi(\cdot): \mathbb{R}^{k\times d}\times \mathbb{R}^{k\times k} \rightarrow \mathbb{R}^{k\times d'}$ takes each subgraph as input, and embeds each node on the input subgraph into a latent representation.
We take the representations of each central node $i$ learned from the original data as $\mathbf{z}_i$, and we use $\mathbf{Z}=\{\mathbf{z}_i\}_{i=1}^n$ for downstream tasks. 
For the sampled counterfactual subgraphs in $\mathcal{\bar{G}}^{(i)}$ and $\mathcal{\underline{G}}^{(i)}$, we use an aggregator (e.g., mean aggregator) $\mathtt{AGG}(\cdot)$ to aggregate the representations of each central node $i$, and obtain the final representations $\mathbf{\bar{z}}_i$ and $\mathbf{\underline{z}}_i$. %The aggregators can be a mean aggregator or pooling aggregators. 

To encode useful information of node features and graph structure into the representations, we use labels as supervision. We use the task of node classification as an example, but our framework can be naturally extended to other kinds of tasks on graph data such as link prediction. We denote the class labels as $\mathbf{Y}=\{y_1,...,y_n\}$ for the $n$ nodes. The prediction loss can be formulated as:
\begin{equation}
    \mathcal{L}_p = \frac{1}{n}\sum\nolimits_{i\in[n]}l(f(\mathbf{z}_i), y_i),
\end{equation}
% \begin{equation}
%     \mathcal{L}_p = \frac{1}{n}\sum\nolimits_{i\in[n]}\frac{1}{3}(l(f(\mathbf{z}_i), y_i)+l(f(\mathbf{\bar{z}}_i), y_i)+l(f(\mathbf{\underline{z}}_i), y_i)),
% \end{equation}
where $l(\cdot)$ is the loss function (e.g., cross-entropy) which measures the prediction error, $f(\cdot)$ makes predictions for downstream tasks with the representations, i.e., $\hat{y}_i=f(\mathbf{z}_i)$. Finally, the overall loss function for fair representation learning is:
\begin{equation}
    \mathcal{L} = \mathcal{L}_p + \lambda\mathcal{L}_f + \mu \|\theta\|^2,
\end{equation}
where $\theta$ is the set of model parameters, $\lambda$ and $\mu$ are hyperparameters controlling the weight of the graph counterfactual fairness constraint, and $L_2$ norm regularization, respectively.

==> fmvmfnbbgqzmgyncbhqsqqzvbvfhfcxv/problem.tex <==
\section{Problem Definition}
\begin{table}[t]
\small
  \caption{Notation.}
  \label{tab:notation}
  \vspace{-4mm}
  \begin{tabular}{ll}
    \toprule
    Notation & Definition \\ 
    \midrule
    $\mathcal{G}$,$\mathcal{V},\mathcal{E}$          & the original graph, the set of vertices/edges \\
    $\mathbf{X},\mathbf{x}_i$ & features of all nodes/the $i$-th node\\
    $\mathbf{A}$          & adjacency matrix\\
    $n$               & the number of nodes \\
    $\mathbf{S},{s}_i$ & sensitive attribute values of all nodes/the $i$-th node\\
    $\mathbf{Z},\mathbf{z}_i$ & representations of all nodes/the $i$-th node\\
    $\Phi(\cdot),\phi(\cdot)$  & encoder/subgraph encoder\\
    $\mathtt{AGG(\cdot)}$  & aggregator \\
    $f(\cdot)$             & downstream classifier/predictor \\
    $(U)_{V \leftarrow v}$ & counterfactual of variable $U$ when $V$ had been set to $v$\\
    $\neg i$          & the indices which are not $i$\\
    $d,d'$               & dimension of features/representations \\
    %$d'$              & dimension of representations \\
    $(\cdot)^{(i)}$   & information of the subgraph with central node $i$ \\
    $\mathtt{SUB}(\cdot)$ & subgraph generation operator \\
    $\mathtt{SMP}(\cdot)$ & sampling operation of sensitive attribute\\
    %$\mathcal{V}^c$   & the set of nodes with counterfactual data \\
    $\tilde{\mathbf{S}}$ & the summary of neighboring sensitive attribute values\\
    $\mathcal{\bar{G}}^{(i)}$,$\mathcal{\underline{G}}^{(i)}$  & the set of counterfactual subgraphs of $\mathcal{G}^{(i)}$ under \\ & self-perturbation/neighbor-perturbation \\
    %&of the sensitive attributes of node $i$\\
    %& the set of counterfactual subgraphs of $\mathcal{G}^{(i)}$ under \\ & \\
    %&of the sensitive attributes of node $i$'s neighbors\\
    %$C_1$           & the number of counterfactual subgraphs generated by \\&perturbation on the sensitive attributes of central nodes\\
    $C$           & the sampling number in neighbor-perturbation\\
    \bottomrule
\end{tabular}
\vspace{-2mm}
\end{table}
% Notations: upper case: matrix, lower case: 
\textbf{Notations.} Given a graph $\mathcal{G}=\{\mathcal{V}, \mathcal{E}, \mathbf{X}\}$, where $\mathcal{V}$ is the set of nodes, $\mathcal{E}$ is the set of edges, $\mathbf{X}=\{\mathbf{x}_i\}_{i=1}^n$ denotes the node features $(n=|\mathcal{V}|)$, and $\mathbf{x}_i \in \mathbb{R}^d$ represents the features of node $i$. $\mathbf{A}\in \mathbb{R}^{n\times n}$ denotes the adjacency matrix of the graph $\mathcal{G}$, where $\mathbf{A}_{i,j}=1$ if edge $i\rightarrow j$ exists, otherwise $\mathbf{A}_{i,j}=0$. Without loss of generalization, we assume $\mathcal{G}$ is undirected and unweighted, but this work can be naturally extended to directed or weighted settings. 
%
Each node $i$ has a sensitive attribute ${s}_i \in \{0, 1\}$ (we assume one single, binary sensitive attribute for simplicity, but our model can also be easily extended to multivariate or continuous sensitive attributes). $\mathbf{S}=\{s_i\}_{i=1}^n$, and ${s}_i$ is included in $\mathbf{x}_i$. We denote the non-sensitive features as $\mathbf{X}^{\neg s}=\{\mathbf{x}^{\neg s}_1,...,\mathbf{x}^{\neg s}_n\}$, where $\mathbf{x}^{\neg s}_i = \mathbf{x}_i \backslash {s}_i$.

% graph representation learning
Traditional node representation learning methods train an encoder  $\Phi(\cdot): \mathbb{R}^{n\times d} \times \mathbb{R}^{n \times n}\rightarrow \mathbb{R}^{n\times d'}$ to map each node to a latent representation. The learned representations for the $n$ nodes are denoted by $\mathbf{Z}=\{\mathbf{z}_i\}_{i=1}^n$, where $\mathbf{z}_i=(\Phi(\mathbf{X},\mathbf{A}))_i$, $\mathbf{z}_i\in \mathbb{R}^{d'}$ for any node $i$, and $d'$ is the dimensionality of node representations. These representations can be used in various downstream tasks like node classification \cite{bhagat2011node}, link prediction \cite{liben2007link}, and graph classification \cite{ying2018hierarchical}. $f(\cdot)$ denotes the downstream classifier/predictor. In the node classification task, let $y_i$ denote the true label of the node $i$, $f(\cdot)$ takes the representation $\mathbf{z}_i$ as input, and outputs the predicted label $\hat{y}_i$.

% fairness
% two kinds of "narrow" definitions: encoder and fairness: 
%     1. the general encoder should consider all X and A, but we usually only need the subgraphs, x_i, x_N(i), A_sub(i)
%     2. the fairness representation should be independent with ALL other nodes in the graph, but here we only consider the subgraphs.
%\noindent\textbf{Fairness in graph representation learning.} Recently, many graph representation learning methods \cite{li2020dyadic,dai2020fairgnn,agarwal2021towards} have incorporated  fairness notions to eliminate the discrimination of the learned representations against certain demographic sensitive subgroups.
%
\noindent\textbf{Counterfactual fairness.} Counterfactual fairness \cite{kusner2017counterfactual} is a fairness notion based on Pearl's structural causal model \cite{pearl2009causal}. A \textit{causal model} consists of  a \textit{causal graph} and \textit{structural equations}. A causal graph is a directed acyclic graph (DAG), where each node represents a variable, and each directed edge represents a causal relationship. Structural equations describe these causal relations among  variables. For variables $Y, S$, the value of the \textit{counterfactual} "what would $Y$ have been if $S$ had been set to $s$?" is denoted by $Y_{S\leftarrow s}$. 
% CF
Based on a given causal model, a predictor $\hat{Y}=f(X)$ is \textit{counterfactually fair} \cite{kusner2017counterfactual} if under any features $X=x$ and sensitive attribute $S=s$, 
\vspace{-1mm}
\begin{equation}
P(\hat{Y}_{S\leftarrow s}=y|X=x,S=s) = P(\hat{Y}_{S\leftarrow s'}=y|X=x,S=s),
\vspace{-1mm}
\end{equation}
for all $y$ and $s'\ne s$. Here $\hat{Y}_{S\leftarrow s}=f(X_{S\leftarrow s},s)$ denotes the prediction made on the counterfactual when $S$ had been set to $s$. Intuitively, it aims to minimize the difference between predictions made on each individual and its counterfactuals with different sensitive attribute values. Ideally, the counterfactuals should be generated based on the ground truth causal model. 
% statistical vs CF, iid data
Different from the statistical fairness notions such as equality of opportunity (EO) \cite{hardt2016equality,zafar2017fairness} and demographic parity (DP) \cite{zemel2013learning}, counterfactual fairness %tracks the generation of biases with the causal model, and 
aims to eliminate the biases led by the causal effect from the sensitive attribute on the observed variables used for model training. % a counterfactually fair predictor. 
However, most existing works of counterfactual fairness focus on i.i.d. data.

\noindent\textbf{Existing notion of counterfactual fairness on graph.} 
%
Recent works \cite{agarwal2021towards,agarwal2021towards2} have extended counterfactual fairness to graphs.   %but most of them are based on %naive
% overly simplified assumptions on the causal model. 
Given a graph $X=\mathbf{X}, A=\mathbf{A}$, these works consider that an encoder $\Phi(\cdot)$ satisfies  counterfactual fairness if for any node $i$:
\vspace{-1mm}
% \begin{equation}
%     (\Phi(\mathbf{X}_{{s}_i= {0}},\mathbf{A}))_i = (\Phi(\mathbf{X}_{{s}_i= {1}},\mathbf{A}))_i,
%     \label{eq:naive_gcf}
%     \vspace{-1mm}
% \end{equation}
\begin{equation}
    (\Phi({X}_{{S}_i={0}},{A}))_i = (\Phi({X}_{{S}_i= {1}},{A}))_i,
    \label{eq:naive_gcf}
    \vspace{-1mm}
\end{equation}
% actual definition is even more naive, when they assume ENC(u) on each node, rather than the whole graph
where ${X}_{{S}_i= {0}}$ and ${X}_{{S}_i= {1}}$ denote the node features after setting $S_i$ as $0$ and $1$, respectively, while everything else does not change\footnote{We use italicized uppercase letters (e.g., $S_i,X,A$) to denote random variables, and use 
italicized lowercase letters (e.g., $s_i$), non-italicized bold lowercase/uppercase letters (e.g., $\mathbf{x}_i$ and $\mathbf{X}$) to denote specific realization of scalars or vectors/matrices, respectively. }.
This notion considers fairness as minimizing the discrepancy between the representations of each node with different values of its sensitive attribute (while everything else is fixed). This notion has the following limitations: 1) %the effect of other nodes' sensitive attributes on the label of each node is not considered as unfair, i.e., the main limitation of this notion is that 
it does not consider the potential biases led by the causal effect from the sensitive attribute of other nodes in the graph on the prediction of each node; 2) it implicitly assumes that the sensitive attribute has no causal effect on other features or the graph structure. 
In a nutshell, this fairness notion is more limited than the general counterfactual fairness notion. %, although it is a good starting point for more general counterfactual fairness metrics for graphs. %Although it is believed that only setting the sensitive attributes itself can capture the most important issues in many prediction tasks [], and
%Intuitively, this fairness notion is satisfied if for any node $i$, the node representation $\mathbf{z}_i$ is independent with its own sensitive attributes. 

% An encoder $\Phi(\cdot): \mathbb{R}^{n\times d} \times \mathbb{R}^{n \times n}\rightarrow \mathbb{R}^{n\times d'}$ satisfies graph counterfactual fairness if for any node $i$: 
% % \begin{equation}
% %     P(\mathbf{z}_i| \mathbf{s}_i=\mathbf{s}, \mathbf{x}^{\neg s}_i, \mathbf{A}_i) = P(\mathbf{z}_i| \mathbf{s}_i=\mathbf{s}', \mathbf{x}^{\neg s}_i, \mathbf{A}_i),
% % \end{equation}
% \begin{equation}
%     (\Phi(\mathbf{X}_{\mathbf{s}_i\leftarrow \mathbf{s}},\mathbf{A}_{\mathbf{s}_i\leftarrow \mathbf{s}}))_i = (\Phi(\mathbf{X}_{\mathbf{s}_i\leftarrow \mathbf{s}'},\mathbf{A}_{\mathbf{s}_i\leftarrow \mathbf{s}'}))_i,
% \label{eq:naive_gcf}
% \end{equation}
% where $\mathbf{s},\mathbf{s'} \in \mathbb{R}^{K}$ are any specific values of sensitive attributes, and in the general ``counterfactual fairness'' notion, the operation $\mathbf{s}_i \leftarrow \mathbf{s}$ means to generate a counterfactual data [] based on a given causal model, but these causal models can hardly be completely obtained, and recent literature [] often generate the counterfactual data by directly setting the sensitive attributes of node $i$, while leave other parts fixed. We denote this operation by $\mathbf{X}_{\mathbf{s}_i= \mathbf{s}}$. Based on this operation, the corresponding fairness notion is defined as:
% \begin{equation}
%     (\Phi(\mathbf{X}_{\mathbf{s}_i= \mathbf{s}},\mathbf{A}))_i = (\Phi(\mathbf{X}_{\mathbf{s}_i= \mathbf{s}'},\mathbf{A}))_i,
% \end{equation}



\noindent\textbf{Graph counterfactual fairness.} To address the above limitations, in this work, we propose a novel fairness notion on graphs: 
\vspace{-2mm}
\begin{definition}
{(Graph counterfactual fairness).}
An encoder $\Phi(\cdot)$ satisfies graph counterfactual fairness if for any node $i$:
\begin{equation}
    P(({Z}_i)_{{S}\leftarrow \mathbf{s}'}|X=\mathbf{X},A=\mathbf{A})=P((Z_i)_{{S}\leftarrow \mathbf{s}''}|X=\mathbf{X},A=\mathbf{A}),
    \label{eq:gcf}
\end{equation}
% \begin{equation}
%     P((\hat{Y}_i)_{{S}\leftarrow \mathbf{s}'}|X=\mathbf{X},A=\mathbf{A})=P((\hat{Y}_i)_{{S}\leftarrow \mathbf{s}''}|X=\mathbf{X},A=\mathbf{A}),
%     \label{eq:gcf}
% \end{equation}
\noindent for all $\mathbf{s}' \!\ne \!\mathbf{s}''$, where $\mathbf{s}', \mathbf{s}''\! \in\! \{0,1\}^{n}$ are arbitrary sensitive attribute values of all nodes, $Z_i=(\Phi(X,A))_i$ denotes the node representations for node $i$. In other words, given a graph $X=\mathbf{X}, A=\mathbf{A}$, $\Phi(\cdot)$  %an encoder $\Phi(\cdot)$ 
%: \mathbb{R}^{n\times d} \times \mathbb{R}^{n \times n}\rightarrow \mathbb{R}^{n\times d'}$ 
%towards graph counterfactual fairness 
should minimize the distribution discrepancy between the representations $(\Phi({X}_{{S}\leftarrow \mathbf{s}'},{A}_{{S}\leftarrow \mathbf{s}'}))_i$ and $(\Phi({X}_{{S}\leftarrow \mathbf{s}''},{A}_{{S}\leftarrow \mathbf{s}''}))_i$ for any node $i$. 
% \begin{equation}
%     (\Phi(\mathbf{X}_{\mathbf{S}\leftarrow \mathbf{s}'},\mathbf{A}_{\mathbf{S}\leftarrow \mathbf{s}'}))_i = (\Phi(\mathbf{X}_{\mathbf{S}\leftarrow \mathbf{s}''},\mathbf{A}_{\mathbf{S}\leftarrow \mathbf{s}''}))_i,
% \label{eq:gcf}
% \end{equation}
% \begin{equation}
% \label{Eq: graphcf}
%     P(\mathbf{z}_i| \mathbf{s}_i=\mathbf{s}, \mathbf{S}_{\neg i}=\mathbf{S}', \mathbf{x}^{\neg s}_i, \mathbf{A}_i) = P(\mathbf{z}_i| \mathbf{s}_i=\mathbf{s}',\mathbf{S}_{\neg i}=\mathbf{S}'', \mathbf{x}^{\neg s}_i, \mathbf{A}_i),
% \end{equation}
% \begin{equation}
% \label{Eq: graphcf}
%     (\Phi(\mathbf{X}_{\mathbf{s}_i= \mathbf{s}, \mathbf{S}_{\neg i}=\mathbf{S}'},\mathbf{A}))_i = (\Phi(\mathbf{X}_{\mathbf{s}_i= \mathbf{s}',\mathbf{S}_{\neg i}=\mathbf{S}''},\mathbf{A}))_i,
% \end{equation}
\end{definition}
%where the subscript $(\cdot)_{\neg i}$ denotes all the other nodes in the graph except node $i$, and $\mathbf{S}', \mathbf{S}'' \in \mathbb{R}^{(n-1)\times K}$ are any specific values of sensitive attributes of other nodes in the graph. This notion can be interpreted as follows: node representations output by encoder $\Phi(\cdot)$ should be independent of the sensitive attributes of all the nodes in the graph. 
%Here,  {$\mathbf{X}_{{S}\leftarrow \mathbf{s}'}$ refers to a specific value of the counterfactual ``what would the node features have been if the sensitive attributes of the $n$ nodes had been set by $s'$, conditioned on the original data, including node features $\mathbf{X}$ and graph structure $\mathbf{A}$?"}
Intuitively, this notion encourages the representations learned from the original graph and counterfactuals to be equal. The counterfactuals correspond to different cases when the sensitive attribute of the $n$ nodes had been set to any values. 
For notation simplicity, in the following sections, we use {$\mathbf{X}_{{S}\leftarrow \mathbf{s}'}$ to denote a specific value of the counterfactual ``what would the node features have been if the sensitive attribute of the $n$ nodes had been set by $\mathbf{s}'$, given the original data, i.e., node features $\mathbf{X}$ and graph structure $\mathbf{A}$?"}.  We also use notation  $\mathbf{A}_{{S}\leftarrow \mathbf{s}'}$ in a similar way.
%and the operation $U_{V\leftarrow v}$ denotes the counterfactual of variable $U$  when variable $V$ had been intervened to a specific value $v$ and the descendant variables of $V$ are taken values based on the intervened value $v$ and the underlying causal model \cite{pearl2009causal}. %, but these causal models can hardly be completely obtained

% KNN-graph CF
% However, the true causal models can hardly be completely obtained, thus the causal effect from the sensitive attribute of other nodes in the graph on the labels, as well as the causal relations among different variables can be complicated, especially when the input graph is large-scale.
% Based on a common observation \cite{hamilton2017inductive,jiao2020sub} that each node is mostly influenced by its nearest neighbors, we can extract a subgraph $\mathcal{G}^{(i)}$ with node features $\mathbf{X}^{(i)}$ and adjacency matrix $\mathbf{A}^{(i)}$ for each node $i$.
% %
% This subgraph extracts the context information of the central node $i$ on $\mathcal{G}$, i.e., the subgraph of $\mathcal{G}$ which only contains the top $k$ neighbors of node $i$ (including itself). 
% These top-$k$ neighbors are usually contained in the $l$-hop neighbors. 
% We assume that the nodes outside the subgraph $\mathcal{G}^{(i)}$ is independent with the features, graph structure and the label/predicted label of node $i$. Considering this, we relax the original graph counterfactual fairness notion in a subgraph-based form:

%Traditional encoders take the whole graph as input, but as discussed in previous graph representation learning works [], it is often unnecessary and not scalable to taking the complete graph as input. Recent studies [] also show that most of the unfair biases are brought by neighboring nodes. Specifically, for each node $i$, we can extract a subgraph $\mathcal{G}^{(i)}$ with node features $\mathbf{X}^{(i)}$ and adjacency matrix $\mathbf{A}^{(i)}$. This subgraph extracts the context information of the central node $i$ on $\mathcal{G}$, i.e., the subgraph of $\mathcal{G}$ which only contains the top $n'$ neighbors of node $i$ (including itself). Considering this, we define a subgraph-based graph counterfactual fairness notion:
% \begin{definition}
% {(Subgraph counterfactual fairness).}
% An encoder $\Phi(\cdot): \mathbb{R}^{n^{s}\times d} \times \mathbb{R}^{n^{s} \times n^{s}}\rightarrow \mathbb{R}^{n^{s}\times d'}$ satisfies subgraph counterfactual fairness if for any node $j$ in $\mathcal{G}^{(i)}$: 
% \begin{equation}
%  \label{Eq: subgraphcf}
%     (\Phi(\mathbf{X}^{(i)}_{\mathbf{S}^{(i)}\leftarrow\mathbf{s}'},\mathbf{A}^{(i)}))_j = (\Phi(\mathbf{X}^{(i)}_{\mathbf{S}^{(i)}\leftarrow\mathbf{s}''},\mathbf{A}^{(i)}))_j,
% \end{equation}
% \end{definition}
% \begin{equation}
% \label{Eq: subgraphcf}
%     (\Phi(\mathbf{X}^{(i)}_{\mathbf{s}_i= \mathbf{s}, \mathbf{S}^{(i)}_{\neg i}=\mathbf{S}'},\mathbf{A}^{(i)}))_i = (\Phi(\mathbf{X}^{(i)}_{\mathbf{s}_i= \mathbf{s}',\mathbf{S}^{(i)}_{\neg i}=\mathbf{S}''},\mathbf{A}^{(i)}))_i,
% \end{equation}
%\noindent where $n^{s}$ is the number of nodes in subgraph $\mathcal{G}^{(i)}$, and $\mathbf{s}',\mathbf{s}'\in \mathbb{R}^{n^{s}}$, the encoder $\Phi(\cdot)$ takes the context subgraph as input, and outputs the node representations on this subgraph. 
%the encoder $\Phi(\cdot):\mathbb{R}^{n' \times d} \times \mathbb{R}^{n' \times n'} \rightarrow \mathbb{R}^{n'\times d'}$ takes the context subgraph as input, and outputs the node representations on this subgraph. 
% elpsilon-sigma

In this work, we aim to develop a framework which learns node representations on graph towards graph counterfactual fairness, and maintains a good prediction performance simultaneously.


==> fmvmfnbbgqzmgyncbhqsqqzvbvfhfcxv/related.tex <==
\vspace{-2mm}
\section{Related Work}
%\noindent\textbf{Fairness.}
% group fairness and counterfactual fairness
%Fairness in machine learning has attracted significant attention recently \cite{verma2018fairness,kwiatkowska1989survey,binns2020apparent}. Among them, group fairness \cite{zemel2013learning,hardt2016equality,zafar2017fairness,dieterich2016compas,chouldechova2017fair} targets on mitigating the discrimination against certain sensitive attributes. %Traditional group fairness includes various notions such as statistical parity \cite{zemel2013learning}, equalized odds \cite{hardt2016equality,zafar2017fairness}, predictive parity \cite{dieterich2016compas}, and calibration \cite{chouldechova2017fair}. 
%Individual fairness \cite{dwork2012fairness,sharifi2019average} aims to give similar predictions to similar individuals.
%Different from these above notions which are based on statistical population, counterfactual fairness \cite{kusner2017counterfactual,russell2017worlds} considers the counterfactual data, which is another version of each individual with different sensitive attributes. Counterfactual fairness incorporates the causal models \cite{pearl2009causal} to model how the discrimination is exhibited. A predictor which satisfies counterfactual fairness for each individual when the probability distribution of the outcome prediction stay the same in the real and the counterfactual data. 

\noindent\textbf{Graph representation learning.}
% GNN, GCN, GAT
Many efforts have been made for graph representation learning \cite{hamilton2020graph,wang2018graphgan,fey2019fast} in recent years. Among them, neural network methods encode the attributes and graph structure %topology of the graphs
into a latent space as representations to capture useful information. %, and optimize the model to encode more useful information of the graphs. 
These methods include the well-known graph convolutional networks (GCNs) \cite{kipf2016semi}, variational graph auto-encoders (VGAE) \cite{kipf2016variational}, GraphSAGE \cite{hamilton2017inductive}, and structural deep network embedding (SDNE) \cite{wang2016structural}. %These methods encode the input graphs into representations with a series of transformations such as convolutional filters, sample and aggregate method.
Recently, subgraph-based methods \cite{jiao2020sub,nguyen2018learning,crouse2019improving} utilize the  correlation between central nodes and their sampled subgraphs to capture regional structure information and improve the model scalability. Despite the success of these methods in different domains, they may exhibit biases against certain sensitive groups.


\noindent\textbf{Fairness on graphs.}
Fairness in machine learning has attracted significant attention recently \cite{verma2018fairness,kwiatkowska1989survey,binns2020apparent}. Typical fairness notions include group fairness  \cite{zemel2013learning,hardt2016equality,zafar2017fairness,dieterich2016compas,chouldechova2017fair}, individual fairness \cite{dwork2012fairness,sharifi2019average}, and counterfactual fairness \cite{kusner2017counterfactual,russell2017worlds,chiappa2019path,wu2019counterfactual}.
% % adversarial learning, fairGNN, counterfactual graph
Recent works \cite{bose2019compositional,buyl2020debayes,dai2020fairgnn,agarwal2021towards,kang2020inform,dong2021individual} %address the issues of fairness
promote fairness 
in node representation learning. Most of works are based on adversarial learning \cite{beutel2017data,zhang2018mitigating}, aiming to prevent the learned representations from accurately predicting the corresponding sensitive attribute. These works focus on removing the statistical dependency between the sensitive attribute and predictions elicited by the learned representations, but do not consider the biases in the features, graph structure or labels due to the causal effect from the sensitive attribute on them. Differently, few works \cite{agarwal2021towards,agarwal2021towards2} extend counterfactual fairness to graphs. % to incorporate causality. 
However, most of these works do not consider the potential biases brought by the sensitive attribute of neighboring nodes, and the %biases led by the
causal effect from the sensitive attribute to other node features and graph structure.
%the causal effect from the sensitive attribute of neighboring nodes on the prediction, as well as the biases led by the causal effect from the sensitive attribute to other node features and graph structure. %Besides,
%most of them are based on simple change of sensitive attribute values of different nodes, without consideration on the causal influence from sensitive attribute to other observed data such as features or graph structure.

%\vspace{-2mm}

